A Study of the Mathematics of Deep Learning

"Deep Learning"/"Deep Neural Nets" is a technological marvel that is now increasingly deployed at the cutting-edge of artificial intelligence tasks. This dramatic success of deep learning in the last few years has been hinged on an enormous amount of heuristics and it has turned out to be a serious mathematical challenge to be able to rigorously explain them. In this thesis, submitted to the Department of Applied Mathematics and Statistics, Johns Hopkins University we take several steps towards building strong theoretical foundations for these new paradigms of deep-learning. In chapter 2 we show new circuit complexity theorems for deep neural functions and prove classification theorems about these function spaces which in turn lead to exact algorithms for empirical risk minimization for depth 2 ReLU nets. We also motivate a measure of complexity of neural functions to constructively establish the existence of high-complexity neural functions. In chapter 3 we give the first algorithm which can train a ReLU gate in the realizable setting in linear time in an almost distribution free set up. In chapter 4 we give rigorous proofs towards explaining the phenomenon of autoencoders being able to do sparse-coding. In chapter 5 we give the first-of-its-kind proofs of convergence for stochastic and deterministic versions of the widely used adaptive gradient deep-learning algorithms, RMSProp and ADAM. This chapter also includes a detailed empirical study on autoencoders of the hyper-parameter values at which modern algorithms have a significant advantage over classical acceleration based methods. In the last chapter 6 we give new and improved PAC-Bayesian bounds for the risk of stochastic neural nets. This chapter also includes an experimental investigation revealing new geometric properties of the paths in weight space that are traced out by the net during the training.

==> Chapters/Chapter_demo.tex <==
% Chapter 1

\chapter{Chapter Title Here} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
\newcommand{\keyword}[1]{\textbf{#1}}
\newcommand{\tabhead}[1]{\textbf{#1}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\file}[1]{\texttt{\bfseries#1}}
\newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

\section{Welcome and Thank You}
Welcome to this \LaTeX{} Thesis Template, a beautiful and easy to use template for writing a thesis using the \LaTeX{} typesetting system.

If you are writing a thesis (or will be in the future) and its subject is technical or mathematical (though it doesn't have to be), then creating it in \LaTeX{} is highly recommended as a way to make sure you can just get down to the essential writing without having to worry over formatting or wasting time arguing with your word processor.

\LaTeX{} is easily able to professionally typeset documents that run to hundreds or thousands of pages long. With simple mark-up commands, it automatically sets out the table of contents, margins, page headers and footers and keeps the formatting consistent and beautiful. One of its main strengths is the way it can easily typeset mathematics, even \emph{heavy} mathematics. Even if those equations are the most horribly twisted and most difficult mathematical problems that can only be solved on a super-computer, you can at least count on \LaTeX{} to make them look stunning.

%----------------------------------------------------------------------------------------

\section{Learning \LaTeX{}}

\LaTeX{} is not a \textsc{wysiwyg} (What You See is What You Get) program, unlike word processors such as Microsoft Word or Apple's Pages. Instead, a document written for \LaTeX{} is actually a simple, plain text file that contains \emph{no formatting}. You tell \LaTeX{} how you want the formatting in the finished document by writing in simple commands amongst the text, for example, if I want to use \emph{italic text for emphasis}, I write the \verb|\emph{text}| command and put the text I want in italics in between the curly braces. This means that \LaTeX{} is a \enquote{mark-up} language, very much like HTML.

\subsection{A (not so short) Introduction to \LaTeX{}}

If you are new to \LaTeX{}, there is a very good eBook -- freely available online as a PDF file -- called, \enquote{The Not So Short Introduction to \LaTeX{}}. The book's title is typically shortened to just \emph{lshort}. You can download the latest version (as it is occasionally updated) from here:
\url{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}

It is also available in several other languages. Find yours from the list on this page: \url{http://www.ctan.org/tex-archive/info/lshort/}

It is recommended to take a little time out to learn how to use \LaTeX{} by creating several, small `test' documents, or having a close look at several templates on:\\ 
\url{http://www.LaTeXTemplates.com}\\ 
Making the effort now means you're not stuck learning the system when what you \emph{really} need to be doing is writing your thesis.

\subsection{A Short Math Guide for \LaTeX{}}

If you are writing a technical or mathematical thesis, then you may want to read the document by the AMS (American Mathematical Society) called, \enquote{A Short Math Guide for \LaTeX{}}. It can be found online here:
\url{http://www.ams.org/tex/amslatex.html}
under the \enquote{Additional Documentation} section towards the bottom of the page.

\subsection{Common \LaTeX{} Math Symbols}
There are a multitude of mathematical symbols available for \LaTeX{} and it would take a great effort to learn the commands for them all. The most common ones you are likely to use are shown on this page:
\url{http://www.sunilpatel.co.uk/latex-type/latex-math-symbols/}

You can use this page as a reference or crib sheet, the symbols are rendered as large, high quality images so you can quickly find the \LaTeX{} command for the symbol you need.

\subsection{\LaTeX{} on a Mac}
 
The \LaTeX{} distribution is available for many systems including Windows, Linux and Mac OS X. The package for OS X is called MacTeX and it contains all the applications you need -- bundled together and pre-customized -- for a fully working \LaTeX{} environment and work flow.
 
MacTeX includes a custom dedicated \LaTeX{} editor called TeXShop for writing your `\file{.tex}' files and BibDesk: a program to manage your references and create your bibliography section just as easily as managing songs and creating playlists in iTunes.

%----------------------------------------------------------------------------------------

\section{Getting Started with this Template}

If you are familiar with \LaTeX{}, then you should explore the directory structure of the template and then proceed to place your own information into the \emph{THESIS INFORMATION} block of the \file{main.tex} file. You can then modify the rest of this file to your unique specifications based on your degree/university. Section \ref{FillingFile} on page \pageref{FillingFile} will help you do this. Make sure you also read section \ref{ThesisConventions} about thesis conventions to get the most out of this template.

If you are new to \LaTeX{} it is recommended that you carry on reading through the rest of the information in this document.

Before you begin using this template you should ensure that its style complies with the thesis style guidelines imposed by your institution. In most cases this template style and layout will be suitable. If it is not, it may only require a small change to bring the template in line with your institution's recommendations. These modifications will need to be done on the \file{MastersDoctoralThesis.cls} file.

\subsection{About this Template}

This \LaTeX{} Thesis Template is originally based and created around a \LaTeX{} style file created by Steve R.\ Gunn from the University of Southampton (UK), department of Electronics and Computer Science. You can find his original thesis style file at his site, here:
\url{http://www.ecs.soton.ac.uk/~srg/softwaretools/document/templates/}

Steve's \file{ecsthesis.cls} was then taken by Sunil Patel who modified it by creating a skeleton framework and folder structure to place the thesis files in. The resulting template can be found on Sunil's site here:
\url{http://www.sunilpatel.co.uk/thesis-template}

Sunil's template was made available through \url{http://www.LaTeXTemplates.com} where it was modified many times based on user requests and questions. Version 2.0 and onwards of this template represents a major modification to Sunil's template and is, in fact, hardly recognisable. The work to make version 2.0 possible was carried out by \href{mailto:vel@latextemplates.com}{Vel} and Johannes Böttcher.

%----------------------------------------------------------------------------------------

\section{What this Template Includes}

\subsection{Folders}

This template comes as a single zip file that expands out to several files and folders. The folder names are mostly self-explanatory:

\keyword{Appendices} -- this is the folder where you put the appendices. Each appendix should go into its own separate \file{.tex} file. An example and template are included in the directory.

\keyword{Chapters} -- this is the folder where you put the thesis chapters. A thesis usually has about six chapters, though there is no hard rule on this. Each chapter should go in its own separate \file{.tex} file and they can be split as:
\begin{itemize}
\item Chapter 1: Introduction to the thesis topic
\item Chapter 2: Background information and theory
\item Chapter 3: (Laboratory) experimental setup
\item Chapter 4: Details of experiment 1
\item Chapter 5: Details of experiment 2
\item Chapter 6: Discussion of the experimental results
\item Chapter 7: Conclusion and future directions
\end{itemize}
This chapter layout is specialised for the experimental sciences, your discipline may be different.

\keyword{Figures} -- this folder contains all figures for the thesis. These are the final images that will go into the thesis document.

\subsection{Files}

Included are also several files, most of them are plain text and you can see their contents in a text editor. After initial compilation, you will see that more auxiliary files are created by \LaTeX{} or BibTeX and which you don't need to delete or worry about:

\keyword{example.bib} -- this is an important file that contains all the bibliographic information and references that you will be citing in the thesis for use with BibTeX. You can write it manually, but there are reference manager programs available that will create and manage it for you. Bibliographies in \LaTeX{} are a large subject and you may need to read about BibTeX before starting with this. Many modern reference managers will allow you to export your references in BibTeX format which greatly eases the amount of work you have to do.

\keyword{MastersDoctoralThesis.cls} -- this is an important file. It is the class file that tells \LaTeX{} how to format the thesis. 

\keyword{main.pdf} -- this is your beautifully typeset thesis (in the PDF file format) created by \LaTeX{}. It is supplied in the PDF with the template and after you compile the template you should get an identical version.

\keyword{main.tex} -- this is an important file. This is the file that you tell \LaTeX{} to compile to produce your thesis as a PDF file. It contains the framework and constructs that tell \LaTeX{} how to layout the thesis. It is heavily commented so you can read exactly what each line of code does and why it is there. After you put your own information into the \emph{THESIS INFORMATION} block -- you have now started your thesis!

Files that are \emph{not} included, but are created by \LaTeX{} as auxiliary files include:

\keyword{main.aux} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

\keyword{main.bbl} -- this is an auxiliary file generated by BibTeX, if it is deleted, BibTeX simply regenerates it when you run the \file{main.aux} file. Whereas the \file{.bib} file contains all the references you have, this \file{.bbl} file contains the references you have actually cited in the thesis and is used to build the bibliography section of the thesis.

\keyword{main.blg} -- this is an auxiliary file generated by BibTeX, if it is deleted BibTeX simply regenerates it when you run the main \file{.aux} file.

\keyword{main.lof} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Figures} section.

\keyword{main.log} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It contains messages from \LaTeX{}, if you receive errors and warnings from \LaTeX{}, they will be in this \file{.log} file.

\keyword{main.lot} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file. It tells \LaTeX{} how to build the \emph{List of Tables} section.

\keyword{main.out} -- this is an auxiliary file generated by \LaTeX{}, if it is deleted \LaTeX{} simply regenerates it when you run the main \file{.tex} file.

So from this long list, only the files with the \file{.bib}, \file{.cls} and \file{.tex} extensions are the most important ones. The other auxiliary files can be ignored or deleted as \LaTeX{} and BibTeX will regenerate them.

%----------------------------------------------------------------------------------------

\section{Filling in Your Information in the \file{main.tex} File}\label{FillingFile}

You will need to personalise the thesis template and make it your own by filling in your own information. This is done by editing the \file{main.tex} file in a text editor or your favourite LaTeX environment.

Open the file and scroll down to the third large block titled \emph{THESIS INFORMATION} where you can see the entries for \emph{University Name}, \emph{Department Name}, etc \ldots

Fill out the information about yourself, your group and institution. You can also insert web links, if you do, make sure you use the full URL, including the \code{http://} for this. If you don't want these to be linked, simply remove the \verb|\href{url}{name}| and only leave the name.

When you have done this, save the file and recompile \code{main.tex}. All the information you filled in should now be in the PDF, complete with web links. You can now begin your thesis proper!

%----------------------------------------------------------------------------------------

\section{The \code{main.tex} File Explained}

The \file{main.tex} file contains the structure of the thesis. There are plenty of written comments that explain what pages, sections and formatting the \LaTeX{} code is creating. Each major document element is divided into commented blocks with titles in all capitals to make it obvious what the following bit of code is doing. Initially there seems to be a lot of \LaTeX{} code, but this is all formatting, and it has all been taken care of so you don't have to do it.

Begin by checking that your information on the title page is correct. For the thesis declaration, your institution may insist on something different than the text given. If this is the case, just replace what you see with what is required in the \emph{DECLARATION PAGE} block.

Then comes a page which contains a funny quote. You can put your own, or quote your favourite scientist, author, person, and so on. Make sure to put the name of the person who you took the quote from.

Following this is the abstract page which summarises your work in a condensed way and can almost be used as a standalone document to describe what you have done. The text you write will cause the heading to move up so don't worry about running out of space.

Next come the acknowledgements. On this page, write about all the people who you wish to thank (not forgetting parents, partners and your advisor/supervisor).

The contents pages, list of figures and tables are all taken care of for you and do not need to be manually created or edited. The next set of pages are more likely to be optional and can be deleted since they are for a more technical thesis: insert a list of abbreviations you have used in the thesis, then a list of the physical constants and numbers you refer to and finally, a list of mathematical symbols used in any formulae. Making the effort to fill these tables means the reader has a one-stop place to refer to instead of searching the internet and references to try and find out what you meant by certain abbreviations or symbols.

The list of symbols is split into the Roman and Greek alphabets. Whereas the abbreviations and symbols ought to be listed in alphabetical order (and this is \emph{not} done automatically for you) the list of physical constants should be grouped into similar themes.

The next page contains a one line dedication. Who will you dedicate your thesis to?

Finally, there is the block where the chapters are included. Uncomment the lines (delete the \code{\%} character) as you write the chapters. Each chapter should be written in its own file and put into the \emph{Chapters} folder and named \file{Chapter1}, \file{Chapter2}, etc\ldots Similarly for the appendices, uncomment the lines as you need them. Each appendix should go into its own file and placed in the \emph{Appendices} folder.

After the preamble, chapters and appendices finally comes the bibliography. The bibliography style (called \option{authoryear}) is used for the bibliography and is a fully featured style that will even include links to where the referenced paper can be found online. Do not underestimate how grateful your reader will be to find that a reference to a paper is just a click away. Of course, this relies on you putting the URL information into the BibTeX file in the first place.

%----------------------------------------------------------------------------------------

\section{Thesis Features and Conventions}\label{ThesisConventions}

To get the best out of this template, there are a few conventions that you may want to follow.

One of the most important (and most difficult) things to keep track of in such a long document as a thesis is consistency. Using certain conventions and ways of doing things (such as using a Todo list) makes the job easier. Of course, all of these are optional and you can adopt your own method.

\subsection{Printing Format}

This thesis template is designed for double sided printing (i.e. content on the front and back of pages) as most theses are printed and bound this way. Switching to one sided printing is as simple as uncommenting the \option{oneside} option of the \code{documentclass} command at the top of the \file{main.tex} file. You may then wish to adjust the margins to suit specifications from your institution.

The headers for the pages contain the page number on the outer side (so it is easy to flick through to the page you want) and the chapter name on the inner side.

The text is set to 11 point by default with single line spacing, again, you can tune the text size and spacing should you want or need to using the options at the very start of \file{main.tex}. The spacing can be changed similarly by replacing the \option{singlespacing} with \option{onehalfspacing} or \option{doublespacing}.

\subsection{Using US Letter Paper}

The paper size used in the template is A4, which is the standard size in Europe. If you are using this thesis template elsewhere and particularly in the United States, then you may have to change the A4 paper size to the US Letter size. This can be done in the margins settings section in \file{main.tex}.

Due to the differences in the paper size, the resulting margins may be different to what you like or require (as it is common for institutions to dictate certain margin sizes). If this is the case, then the margin sizes can be tweaked by modifying the values in the same block as where you set the paper size. Now your document should be set up for US Letter paper size with suitable margins.

\subsection{References}

The \code{biblatex} package is used to format the bibliography and inserts references such as this one \parencite{Reference1}. The options used in the \file{main.tex} file mean that the in-text citations of references are formatted with the author(s) listed with the date of the publication. Multiple references are separated by semicolons (e.g. \parencite{Reference2, Reference1}) and references with more than three authors only show the first author with \emph{et al.} indicating there are more authors (e.g. \parencite{Reference3}). This is done automatically for you. To see how you use references, have a look at the \file{Chapter1.tex} source file. Many reference managers allow you to simply drag the reference into the document as you type.

Scientific references should come \emph{before} the punctuation mark if there is one (such as a comma or period). The same goes for footnotes\footnote{Such as this footnote, here down at the bottom of the page.}. You can change this but the most important thing is to keep the convention consistent throughout the thesis. Footnotes themselves should be full, descriptive sentences (beginning with a capital letter and ending with a full stop). The APA6 states: \enquote{Footnote numbers should be superscripted, [...], following any punctuation mark except a dash.} The Chicago manual of style states: \enquote{A note number should be placed at the end of a sentence or clause. The number follows any punctuation mark except the dash, which it precedes. It follows a closing parenthesis.}

The bibliography is typeset with references listed in alphabetical order by the first author's last name. This is similar to the APA referencing style. To see how \LaTeX{} typesets the bibliography, have a look at the very end of this document (or just click on the reference number links in in-text citations).

\subsubsection{A Note on bibtex}

The bibtex backend used in the template by default does not correctly handle unicode character encoding (i.e. "international" characters). You may see a warning about this in the compilation log and, if your references contain unicode characters, they may not show up correctly or at all. The solution to this is to use the biber backend instead of the outdated bibtex backend. This is done by finding this in \file{main.tex}: \option{backend=bibtex} and changing it to \option{backend=biber}. You will then need to delete all auxiliary BibTeX files and navigate to the template directory in your terminal (command prompt). Once there, simply type \code{biber main} and biber will compile your bibliography. You can then compile \file{main.tex} as normal and your bibliography will be updated. An alternative is to set up your LaTeX editor to compile with biber instead of bibtex, see \href{http://tex.stackexchange.com/questions/154751/biblatex-with-biber-configuring-my-editor-to-avoid-undefined-citations/}{here} for how to do this for various editors.

\subsection{Tables}

Tables are an important way of displaying your results, below is an example table which was generated with this code:

{\small
\begin{verbatim}
\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}
\end{verbatim}
}

\begin{table}
\caption{The effects of treatments X and Y on the four groups studied.}
\label{tab:treatments}
\centering
\begin{tabular}{l l l}
\toprule
\tabhead{Groups} & \tabhead{Treatment X} & \tabhead{Treatment Y} \\
\midrule
1 & 0.2 & 0.8\\
2 & 0.17 & 0.7\\
3 & 0.24 & 0.75\\
4 & 0.68 & 0.3\\
\bottomrule\\
\end{tabular}
\end{table}

You can reference tables with \verb|\ref{<label>}| where the label is defined within the table environment. See \file{Chapter1.tex} for an example of the label and citation (e.g. Table~\ref{tab:treatments}).

\subsection{Figures}

There will hopefully be many figures in your thesis (that should be placed in the \emph{Figures} folder). The way to insert figures into your thesis is to use a code template like this:
\begin{verbatim}
\begin{figure}
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}
\end{verbatim}
Also look in the source file. Putting this code into the source file produces the picture of the electron that you can see in the figure below.

\begin{figure}[th]
\centering
\includegraphics{Figures/Electron}
\decoRule
\caption[An Electron]{An electron (artist's impression).}
\label{fig:Electron}
\end{figure}

Sometimes figures don't always appear where you write them in the source. The placement depends on how much space there is on the page for the figure. Sometimes there is not enough room to fit a figure directly where it should go (in relation to the text) and so \LaTeX{} puts it at the top of the next page. Positioning figures is the job of \LaTeX{} and so you should only worry about making them look good!

Figures usually should have captions just in case you need to refer to them (such as in Figure~\ref{fig:Electron}). The \verb|\caption| command contains two parts, the first part, inside the square brackets is the title that will appear in the \emph{List of Figures}, and so should be short. The second part in the curly brackets should contain the longer and more descriptive caption text.

The \verb|\decoRule| command is optional and simply puts an aesthetic horizontal line below the image. If you do this for one image, do it for all of them.

\LaTeX{} is capable of using images in pdf, jpg and png format.

\subsection{Typesetting mathematics}

If your thesis is going to contain heavy mathematical content, be sure that \LaTeX{} will make it look beautiful, even though it won't be able to solve the equations for you.

The \enquote{Not So Short Introduction to \LaTeX} (available on \href{http://www.ctan.org/tex-archive/info/lshort/english/lshort.pdf}{CTAN}) should tell you everything you need to know for most cases of typesetting mathematics. If you need more information, a much more thorough mathematical guide is available from the AMS called, \enquote{A Short Math Guide to \LaTeX} and can be downloaded from:
\url{ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf}

There are many different \LaTeX{} symbols to remember, luckily you can find the most common symbols in \href{http://ctan.org/pkg/comprehensive}{The Comprehensive \LaTeX~Symbol List}.

You can write an equation, which is automatically given an equation number by \LaTeX{} like this:
\begin{verbatim}
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}
\end{verbatim}

This will produce Einstein's famous energy-matter equivalence equation:
\begin{equation}
E = mc^{2}
\label{eqn:Einstein}
\end{equation}

All equations you write (which are not in the middle of paragraph text) are automatically given equation numbers by \LaTeX{}. If you don't want a particular equation numbered, use the unnumbered form:
\begin{verbatim}
\[ a^{2}=4 \]
\end{verbatim}

%----------------------------------------------------------------------------------------

\section{Sectioning and Subsectioning}

You should break your thesis up into nice, bite-sized sections and subsections. \LaTeX{} automatically builds a table of Contents by looking at all the \verb|\chapter{}|, \verb|\section{}|  and \verb|\subsection{}| commands you write in the source.

The Table of Contents should only list the sections to three (3) levels. A \verb|chapter{}| is level zero (0). A \verb|\section{}| is level one (1) and so a \verb|\subsection{}| is level two (2). In your thesis it is likely that you will even use a \verb|subsubsection{}|, which is level three (3). The depth to which the Table of Contents is formatted is set within \file{MastersDoctoralThesis.cls}. If you need this changed, you can do it in \file{main.tex}.

%----------------------------------------------------------------------------------------

\section{In Closing}

You have reached the end of this mini-guide. You can now rename or overwrite this pdf file and begin writing your own \file{Chapter1.tex} and the rest of your thesis. The easy work of setting up the structure and framework has been taken care of for you. It's now your job to fill it out!

Good luck and have lots of fun!

\begin{flushright}
Guide written by ---\\
Sunil Patel: \href{http://www.sunilpatel.co.uk}{www.sunilpatel.co.uk}\\
Vel: \href{http://www.LaTeXTemplates.com}{LaTeXTemplates.com}
\end{flushright}


==> Useless/Acknowledgement.tex <==

Sometime in Fall 2015, I landed at Prof. Amitabh Basu's office as a jobless, penniless and homeless grad student looking for a fresh start in life while on leave from my previous physics grad school and my immigration documents being in a complete mess. My JHU story started in the middle of me giving up on academics as a whole. Only a couple of weeks before I had that out-of-the-blue meeting with my adviser Prof. Amitabh Basu, I was essentially putting up in a room in the attic of my friend Dr. Pooja Tyagi and her husband Dr. Lars Grant in the suburbs of Urbana-Champaign - because my lease there had run out and without a job I couldn't have rented a new place. 

An year before this fortuitous meeting with Prof. Amitabh Basu, I was a jobless guy sharing a room with a bunch of strangers in a seedy hotel in a dark alley of Bangalore, India. I was roaming around the city trying to meet scientists there. (Long back during my undergrad I had once landed in Bangalore at the ``National Centre for Biological Sciences (NCBS)" looking to attend a conference on evolutionary biology - while I was considering doing that for research!) It was during these random travels in summer 2014 that I landed a meeting with the legendary mathematician Prof. Nikhil Srivastava (now at UC Berkeley) who was then at Microsoft Research, Bangalore. It was Prof. Nikhil Srivastava, who over lunch gave me the final push to switch paths away from physics and start doing mathematics full-time. Most critically Prof. Nikhil Srivastava got me a TA position with Prof. Alexandra Kolla in the Computer Science department of UIUC. (I do not think that ever before this the CS department of UIUC had ever hired a physics student as a TA! On many days I would read up multiple chapters of the book by Cormen, Leiserson, Rivest and Stein to be able to teach the undergrad class the next day!) 

This arrangement with Prof. Alexandra Kolla, gave me a funding mechanism which I used to take up every advanced course in theoretical CS that was on offer at UIUC and via participating in the research meetings with her I got my first glimpse of what ``applied mathematics" looks like! Before this I had never seen anything about algorithms and invariably I bombed at the mid-semester exam of the extremely advanced graduate algorithms course of UIUC that I had taken up.
But with enormous effort I managed to pass that course and mustered up the courage to register for the graduate complexity theory course that was being taught by Prof. Mahesh Vishwanathan. That was indeed a turning point given how much I enjoyed the subject compared to almost everything that I had studied before this. Prof. Mahesh kept encouraging me and he kept me going through thick and thin. I shall forever be indebted to Prof. Mahesh Vishwanathan for agreeing to write letters of recommendation for this complete outsider that I was and for so critically helping me restart a career outside physics!

I stumbled into deep-learning while I randomly went to NYC to attend a conference on the same while not even knowing what a neural net is. The first time I listened to the talks, particularly by Prof. Anna Choromanska (NYU), on what the theoretical puzzles here are, I was somehow very strongly reminded of the nature of questions in String Theory that I so wanted to pursue while in physics. 

It was only much later that I came to know of the startling fact that arguably neural nets can be said to have majorly pioneered in Johns Hopkins University itself thanks to the series of historic papers that were co-authored by the living legend Terrence J. Sejnowski between 1983-1986, when he was at the Johns Hopkins University, {\tt Analyzing Cooperative Computation} (with Geoffrey E. Hinton), {\tt Optimal Perceptual Inference} (with Geoffrey E. Hinton), {\tt Boltzmann Machines : Constraint Satisfaction Networks That Learn} (with Geoffrey E. Hinton and David H. Ackley) and {\tt A Learning Algorithm for
Boltzmann Machines} (with Geoffrey E. Hinton and David H. Ackley). It definitely comforting me to be able to connect to this interesting piece of history that much of the foundational ideas about neural nets were essentially invented in JHU - something that I have never found mentioned enough in my neighbourhood.

Possibly the single-most interesting idea in all of physics that had always captivated my imagination was the story of Large-N Matrix Models : a beautiful mathematical construction which is prima-facie a Quantum Field Theory but mysteriously enough it has time and again been shown to encode critical features of also being a gravitational theory and it has also been known to be a framework for addressing various deep questions in algebraic geometry. I so much wanted to pursue this subject in the physics department and yet that opportunity never arrived. Maybe deep down one of the things that got me motivated about deep-learning is its superficial resemblance to Matrix Models in physics - and I do hope that someday we will be able to figure out a robust connection between the two. Many a days in grad-school, I woke up in the morning feeling depressed about not being able to do this research. It didn't help that during my Ph.D., the storm of Jackiw-Teitelboim gravity started blowing over physics : which is yet another exciting avatar of Matrix Models. It took a lot of psychological effort on my part to not disband all my ongoing thesis work and dive into this development which was clearly looking to be so much more exciting! On my table, I have always had open a copy of Marcos Marino's lectures on this topic - hoping if someday I could finally get to thinking about these beautiful questions. 

Long back I used to research in Quantum Field Theory with Prof. Shiraz Minwalla and in retrospect I don't think I had been fully conscious of the ``magic" of how he works and thinks. His abilities are legendary about being able to intuit the essential characteristics of the answer bypassing the apparent complexity of the equations. It was only during my Ph.D. when I started to think of research ``$24\times7$" that I finally began to realize all the intangible things that I had actually learnt from him - which went a lot beyond the mechanics of the homotopy based classification of instantons and solitons that he had taught me as an undergrad. Deeper I went into research more I realized as to how profoundly had Prof. Shiraz Minwalla moulded my psyche and approach towards research.  

In this respect I need to also mention the profound influence that Prof. S. Ramanan had on me as an undergrad. I can trace back to say that my interest in research level mathematics essentially started with his evening classes whereby he taught a bunch of us undergrads (at the Chennai Mathematical Institute) from his renowned book ``Global Calculus". In retrospect it seems incredible that he was able to devise a way to teach us beginning undergrads about sheaf theory and Dolbeault cohomology. Prof. S. Ramanan instilled in me a sense of adventure and courage about doing mathematics which continues to shape how I think! 

On almost half the days I found it difficult to motivate myself to come to work. But everyday I put up this fight against depression to get myself to the institute. Probably being able to systematize this was one of the biggest struggles I ``won" during my Ph.D. - that I figured out a mental gymnastics routine to be able to do my usual 10 {\rm AM}-10{\rm PM} schedule of work everyday despite an almost persistent feeling of sadness. This struggle against a perpetually imminent emotional collapse was far harder than the struggle with any mathematics question that I tried during my grad-school.  

I often feel that maybe the only talent I have is my ability to get a certain amount of mathematics done despite these drowning feelings. The situation was essentially caused and continuously exacerbated by my increasing levels of academic loneliness and absence of shared interests with people around. Another factor that has been constantly gnawing at me from inside is that my current path has been causing a fast erosion of my previous geometric studies since nothing I do now is related to the kind of mathematics that I was pursuing before starting grad-school, like studying Riemann surfaces. I am hoping that sometime in future I shall be able to connect back to that path!  

I have never really liked going to classes and sitting through courses. Hence it became a huge struggle to maintain my scientific enthusiasm against the tide of the usual rigmarole of grad-school that seemed to be heavily weighing me down. I guess, I do not have any of the socially expected characteristics of being an ``academic" and the process of Ph.D. has left me entirely conflicted between this realization and my intrinsic energy to relentlessly pursue the research questions that interest me. I do not yet know whether I can be a researcher or whether, if at all anywhere, I fit into the panoply of academia. 

It is to be noted here as to how much my career was affected by Prof. Mauro Maggioni's course titled, ``High-Dimensional Approximation, Probability, and Statistical Learning" It was definitely a turning point in my journey. I had come into grad school with neither any knowledge nor any inclination towards anything in probability theory or statistics. I had almost never found anything interesting about these subjects but as it turns out that its impossible to do deep-learning theory without these. This course by Prof. Mauro Maggioni immensely helped me see probability theory through a more familiar lens of geometry. This course gave me a psychological bridge between a form of thinking which was natural to me and the new terrain of probability theory which I had to get comfortable with to make progress with deep-learning. Prof. Mauro Maggioni introduced me to this book by Roman Vershynin, ``High-Dimensional Probability" and that eventually became a pivot for all of my graduate studies. This book was a starting point from which I launched into reading other similar writings by Phillip Rigollet and Roman Handel that are getting increasingly read by contemporary researchers in this field. I went on to do all the courses that Prof. Mauro Maggioni ever offered! 

In this context I need to express my immense gratitude towards Prof. Laurent Younes, not only for his careful reading of my thesis but also for checking some of my results even during the course of my studies. His readings have led to at least two major changes in my papers and no words can express how much I am grateful to him for these two significant contributions that he has made to my research.  

The last two and a half years were essentially just me sitting in some corner of the institute scribbling away at questions which I could not get anyone I knew motivated about. I tried meeting anyone I thought who might have some overlap with stuff I was getting excited about but I essentially failed to convince almost everyone about the merits in my directions. This complete emotional failure eventually became the defining characteristic of my Ph.D. journey. It was a situation of complete despair and I never found a solution to it, except to learn to accept the desolation. I am very far from being a ``scientist in the attic" and I think I thrive the most in collaborative atmospheres, while brainstorming freely with others for hours. Given this natural emotional disposition of mine, the process of getting a Ph.D. seemed to be happening in an atmosphere entirely antithetical to whatever feels natural or comfortable to me. Research seems to firstly be a challenge of survival in solitary confinement. Almost everyday I have doubted if I could have continued doing this for even one more day unless something dramatically changed about this situation. 

I am enormously grateful to two of my grad student peers, Akshay Rangamani and Ramchandran Muthukumar, who at various points for short periods of time had a lot of regular meetings with me and wrote papers with me. The process of brainstorming with them was one of the few things that kept me stable through those periods. Likewise Soham De (then a grad student at the University of Maryland, now at DeepMind, UK) and co-grad student Pushpendre Rastogi were two other incredible peers from the experimental deep-learning community who spent an enormous amount of time chasing down ideas with me. In the process they taught me a whole lot of things about how deep-nets behave - things I could have only learnt by poring through experimental data with them! There were very many others in JHU, discussions with whom have contributed to my thinking : Enayat Ullah, Prof. Raman Arora, Prof. Trac Tran, Prof. Rene Vidal, Joseph Paat, Prof. James Spall, Prof. Daniel Robinson and Prof. Jeremias Sulam. 

Almost every month I have thought of changing my research direction to something more mainstream in the campus, in hope if doing so would get me more human interactions and discussions. But as much as I desperately struggled to find collaborations and brainstorming sessions with others in the campus, I couldn't ignore the fact that I was deeply attracted to the questions of deep-learning theory. The spectacular progress the subject was making in the world outside was what kept me inspired and yet it was this same attraction which made my loneliness entirely untenable. I personally feel that it was almost a miracle that I could continue doing some research despite the tremendous emotional strain I found myself in. For reasons not entirely clear to me, in this process I often came to appreciate the famous quote by Albert Camus, ``The only way to deal with an unfree world is to become so absolutely free that your very existence is an act of rebellion."  

It is hard to underestimate how much social media like Twitter and Facebook have contributed to deep-learning theory. These have phenomenally impacted the subject not just in terms of actually funding such research but also via the volume of high-quality discussions on these topics that happens between the experts on those platforms. Often my only way of getting to know what the most exciting directions in the community were, was via keeping track of the discussions on the Twitter threads between the luminaries in the field! This is essentially how I found my post-doc position with the renowned mathematician in the field, Prof. Weijie Su at Wharton, UPenn! 

It was also through such social networks that I became aware of Prof. Dan Roy's works and thanks to his kindness I landed an internship with him at the Vector Institute of Artificial Intelligence at UToronto. That was an eye-opening experience which not only got me the last chapter of this thesis but it also got me introduced to a high-voltage learning theory atmosphere in Vector - something quite unlike whatever I had ever experienced before! But maybe more than that, the couple of months I spent attending Prof. Dan Roy's group meetings got me introduced to this exciting subject of ``Stochastic Differential Equations (SDEs)". It was a gust of fresh air, which in my ways fundamentally altered my research thinking. As far as I can forsee the interface between SDEs and deep-learning is going to be a focal point of my works in the coming months! In this context I need to express my immense gratitude for Prof. Avanti Athreya in the department who patiently answered many of my questions about SDEs and thus further propelled my interest in this field. 

It was also though social media that I came to interact with seniors in the field like Prof. Animashree Anandkumar (Caltech) and Prof. Lalitha Sankar (ASU). I shall be immensely grateful for the amount of encouragement that Prof. Lalitha Sankar provided me in my journey through the last couple of years. Many a days were lit up by virtue of her kind words. Also an equal amount of thanks is to due to Kenji Kawaguchi (then a grad student at MIT and now a faculty at NUS), Prof. Chinmay Hegde (NYU) and Prof. Rajarshi Mukherjee (Harvard) who have had extensive brain-storming sessions with me on various deep-learning questions and I hope that some of the ideas from these meetings will see the light of the day in near future.  It is also to be noted as to how much Prof. Kazi Rajibul Islam at UWaterloo inspired me to write an introductory article on deep-learning targeted towards undergrads and high-school students.  He read and edited various drafts that I wrote for this purpose and eventually that became the chapter in my thesis that has been titled, ``An Informal Introduction to Deep-Learning". Prof. Kazi Rajibul Islam also arranged to get it translated into Bangla by Dr. Amiya K. Maji at the Purdue University. They have in turn helped disseminate the translation into a wider audience via their web-portal Bigyan.org.in

Despite these sporadic sparks of inspiration from the outside world, eventually it became very hard to not think of graduate school like a ``zero-sum game" - as understood colloquially. The emotional burnout and other losses in life seemed to compound so massively that ultimately it became hard for me to see any bigger point in the process than just wanting this degree which happens to be a qualification cut-off for certain jobs I would like to be able to get someday. A whole lot thanks is to due to co-grad student Aarushi Goel, who helped many a days by volunteering to play badminton with me or by just sitting around listening to me. This emotionally excruciating process of going through grad school has taken a lot of toll on my family members who have stood through thick and thin with me : my mother Dr. Suranjana Sur, my maternal grand-mother Mira Sur, my sister Subhalakshmi, my aunt Debanjana Bhattacharyya, my cousin sister Debadrita Bhattacharyya and my uncle Dibyendu Bhattacharyya.

%\newpage 
As I end my Ph.D. journey I feel an increasing need to go back to my roots to rediscover the things that really got me started into doing science at all. I began my undergrad studies reading Richard Feynman's famous lectures in physics and as I submit this thesis I find increased resonance in these words of his - which probably I had not begun to appreciate untill now,

\begin{center}
{\color{firebrick}\bf ``We find that the statements of science are not of what is true and what is not true, but statements of what is known to different degrees of certainty. Every one of the concepts of science is on a scale graduated somewhere between, but at neither end of, absolute falsity or absolute truth."}
\vspace{0.3cm}
\linebreak \linebreak 
- Richard Feynman

\vspace*{0.50\textheight}

\begin{center}
{\itshape \color{violet} \fontsize{20}{15}A special thanks is due to Zachary Lubberts and Sayan Chakraborty for helping me set up this LaTeX template for the thesis!}
\end{center}
\end{center}

==> Useless/CV.tex <==
\chapter*{Curriculum Vitae}
\addcontentsline{toc}{chapter}{Curriculum Vitae} 
%\usepackage{koma-moderncvclassic}
\section*{Education}

%>{\centering\arraybackslash}l{0.75\linewidth}


\begin{table}[H]
    %\centering
    \begin{tabular}{r p{12cm}}
        \quad \quad \quad {Fall 2020-} &{Post-Doctoral Researcher at UPenn (Wharton), Statistics with Prof. Weijie Su}{}{}{}{}~\\
    
        \quad \quad \quad Spring 2016 {&{ Ph.D. student (Research Assistant) at the Department of Applied Mathematics}~\\ 
        \quad \quad \quad -Spring 2020 &and Statistics,{ Johns Hopkins University (JHU)},~\\ 
        &{\tt Adviser :} Prof. Amitabh Basu }{}{}{}~\\
        
        \quad \quad \quad {Fall 2011} &{ Graduate student (Physics)}{ University of Illinois at Urbana-Champaign}~\\
        \quad \quad \quad -Spring 2015 & (UIUC){}{{\tt (Starting Fall $2014$ I was a TA in the CS, UIUC department)}}{}~\\
        
        \quad \quad \quad {2008-2011} &{Masters of Science (Physics)}{ Tata Institute of Fundamental Research (TIFR)}{}{}{}~\\
        \quad \quad \quad {2005-2008} &{Bachelor of Science (Hons.)}{ Chennai Mathematical Institute (CMI)}{}{}{}
    \end{tabular}
\end{table}

%\newpage 
\subsection*{Internships}
\begin{tabular}{r p{12cm}}
\quad \quad \quad {June-August $2019$} &{\bf Research Intern }{\bf Adobe Research in San Jose }{Worked with Prof. Sridhar Mahadevan and Anup Rao on distribution free training of deep-nets}{}{}\\ 
\quad \quad \quad {July-August $2018$} &{\bf Research Intern }{\bf Vector Institute For Artificial Intelligence, UToronto }{Work with Prof. Dan Roy on PAC-Bayesian and compression based approaches to proving neural risk bounds}{}{}
\end{tabular}


%\begin{center} 
\newpage 
%\begin{minipage} 
%\vspace{\textheight}


\section*{Research Awards}
    \begin{tabular}{r p{12cm}}
\quad \quad \quad{ITA 2020}&{\bf ``ITA Sea Award'' in recognition of the talk delivered at the conference in the ``Graduation Day" track.}{}{}{}{}\\
\quad \quad \quad{JHU}&{\bf Walter L. Robb Fellowship for 2018-2019}{}{}{}{}\\
\quad \quad \quad{JHU}&{\bf Mathematical Institute for Data Science (MINDS) Fellowship for 2019-2020}{}{}{}{}
    \end{tabular}



\section*{Professional Service} 
\begin{tabular}{r p{12cm}}
\quad \quad \quad{Journal reviewer} &{IEEE Transactions on Pattern Analysis and Machine Intelligence,\newline IEEE Signal Processing Magazine, Neural Computation}{}{}{}{}\\
\quad \quad \quad{Reviewer}&{COLT 2019, AISTATS 2018-2019, ICML 2020 \newline NeurIPS 2018-19 (``top 50\%" reviewer recognition), ICLR 2019}{}{}{}{}\\
\quad \quad \quad{Program committee }&{AAAI-2020, ICML 2018 : Modern Trends in Nonconvex Optimization for Machine Learning, NeurIPS 2019 : Machine Learning with Guarantees}{}{}{}{}\\
\quad \quad \quad{Session chair }&{INFORMS 2020 : Session on Deep Learning Theory and Causal Inference}{}{}{}{}\\

\quad \quad \quad{Societies}&{Institute sponsored student member for $2018-2020$ to the ``Association for Women in Mathematics"}{}{}{}{}
\end{tabular}



%\end{center} 
%\end{minipage} 


% \section*{Working Papers}
% {\small
% \begin{table}[H]
% \begin{tabular}{r p{12cm}}
% \quad \quad \quad {}{{\color{firebrick}``Understanding neurally generated distributions"}}{ with Manuj Mukherjee }{}{}{}
% \quad \quad \quad {}{{\color{firebrick}``Understanding adversarial examples via the output-input Jacobian of nets"}}{ with Jiao }{}{}{}
% \end{tabular}
% \end{table}
% }




\section*{Completed Papers}

 
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
 \quad \quad \quad {\href{https://scholar.google.com/citations?user=V32KjH0AAAAJ&hl=en}{\color{violet}(link)}} &{Google Scholar Profile}{}{}{}{}\\
 
 \quad \quad \quad {\href{https://arxiv.org/abs/2005.04211}{{\color{violet}(link)}}} &{(arXiv:2005.04211)  ``A Study of Neural Training with Non-Gradient and Noise Assisted Gradient Methods''} {}{with Ramchandran Muthukumar}{}{}{}\\
 
 \quad \quad \quad {\href{https://arxiv.org/abs/2005.01699}{{\color{violet}(link)}}}&{(arXiv:2005.01699)  ``Guarantees on Learning Depth-2 Neural Networks Under a Data Poisoning Attack''} {}{with Ramchandran Muthukumar}{}{}{}\\
 
 \quad \quad \quad {\href{https://drive.google.com/file/d/1yhHMX1ROuqRN-_ngAzZGRycjPct0At2e/view?usp=sharing}{\color{violet}(link)}} &{``Improving PAC-Bayesian risk bounds on deep nets using geometrical properties of the training algorithm''}{\color{blue} ICML 2019 Workshop, Understanding and Improving Generalization in Deep Learning}{with Pushpendre Rastogi, Dan Roy (Vector, UToronto) and Jun Yang (Vector, UToronto)}{}{}\\
 
 {\href{https://drive.google.com/file/d/16KHtErsPVgPFl-haebnOWsRffBAYbPEc/view?usp=sharing}{\color{violet}(link)}} &{(arXiv:1807.06766)``Convergence guarantees for RMSProp and ADAM in non-convex optimization and an empirical comparison to Nesterov acceleration''}{{\color{blue}ICML 2018 Workshop, Modern Trends in Nonconvex Optimization for Machine Learning}}{with Soham De (UMD), Enayat Ullah}{}{}\\

\quad \quad \quad{\href{https://eccc.weizmann.ac.il/report/2017/190/}{{\color{violet}(link)}}}&{(ECCC/TR-17/190) ``Lower bounds over Boolean inputs for deep neural networks with ReLU gates''}{with Amitabh Basu}{}{}{}\\


\quad \quad \quad{\href{https://arxiv.org/abs/1708.03735}{{\color{violet}(link)}}} &{(arXiv:1708.03735)  ``Sparse coding and Autoencoders''}{ {\color{blue} IEEE International Symposium on Information Theory (ISIT), 2018} {\color{black} and} {\color{blue} NIPS 2017 workshop on ``Deep Learning : Bridging Theory and Practice"} carry variations of this \href{https://www.overleaf.com/read/zrckrkjwpkrh}{{\color{violet}[ link ]}} shorter version of this otherwise long calculation}{with Akshay Rangamani, Amitabh Basu, Tejaswini Ganapathy (Salesforce, San Francisco), Ashish Arora, Trac D.Tran, Sang (Peter) Chin (BU)}{}{}\\

\quad \quad \quad{\href{https://eccc.weizmann.ac.il/report/2017/098/}{{\color{violet}(link)}}} &{(ECCC/TR-17/098)  ``Understanding Deep Neural Networks with Rectified Linear Units''} {{\color{blue}  International Conference on Learning Representations (ICLR), 2018}}{with Raman Arora, Amitabh Basu and Poorya Mianjy}{}{}{}\\

\quad \quad \quad{\href{http://arxiv.org/abs/1512.01226}{{\color{violet}(link)}}} &{(arXiv:1512.01226) ``Renyi entropy of the critical O(N) model''}{}{}{}{}\\

\quad \quad \quad{\href{https://arxiv.org/abs/1307.7714}{{\color{violet}(link)}}} &{(arXiv:1307.7714) ``n-point correlations of dark matter tracers : Renormalization with univariate biasing and its $O(f_{NL})$ terms with bivariate biasing''}{}{}{}{}
 \end{tabular}
\end{table}
 
 \section*{Major exploratory projects undertaken before coming to JHU}
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
% \quad \quad \quad {JHU} &{{\bf Circuit Complexity}}{ We construct proofs to establish relative approximation hardness between different ReLU circuits. (over real and Boolean domains)}{}{}{}\\

% \quad \quad \quad {} &{{\bf Mathematics of Deep Learning}}{ We are building rigorous proofs in the following major themes : (a) explaining deep-net generalization by blending compression and PAC-Bayesian approaches, (b) the power of adaptive gradient descent and non-gradient methods in being able to train deep nets and (c) the reasons why the neural net landscape can often encode certain classic generative models like sparse-coding.}{}{}{}\\

\quad \quad \quad {UIUC} &{{\tt Ramanujan expanders,}} {We developed deterministic polynomial time heuristics to construct optimal spectral expanders.}{\href{https://www.overleaf.com/read/vtbgmtxpsdmp}{{\color{violet}[Link to the research notes and expository surveys that we have written]}}}{}{}{}~\\
\quad \quad \quad {TIFR} &{{\tt Supersymmetry},}{ I contributed to a paper on the single particle spectrum of {\cal N} = 3 superconformal Chern-Simons's theories with adjoint and fundamental matter in the large $N_c$ limit.}{}{}{}~\\
\end{tabular}
\end{table}


\section*{Invited conference talks}
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
\quad \quad \quad {$6^{th}$ May 2020}&{(postponed)}{ SIAM Conference on Mathematics of Data Science 2020}{}{}{}{}{}\\
\quad \quad \quad {$5^{th}$ Feb 2020}&{\bf ``Graduation Day" talk at the 2020 Information Theory and Applications Workshop}{}{}{}{}{}\\
\quad \quad \quad {$20^{th}$ Oct 2019}&{\bf (2 talks) INFORMS Annual Meeting 2019, Seattle}{}{}{}{}{}\\
\quad \quad \quad {$4^{th}$ Nov 2018}&{\bf INFORMS Annual Meeting 2018, Phoenix}{}{}{}{}{}\\
\quad \quad \quad {$9^{th}$ Jul. 2018}&{\bf SIAM Annual Meeting 2018, Portland}{}{}{}{}{}\\
\quad \quad \quad {$1^{st}$ Jul 2018}&{\bf $23^{rd}$ International Symposium on Mathematical Programming (ISMP) (Bordeux, France)}{}{}{}{}{}\\
\quad \quad \quad {$17^{th}$Aug 2017}&{\bf "Modeling and Optimization: Theory and Applications" (MOPTA) 2017}{}{}{}{}{}
\end{tabular}
\end{table}

\section*{Talks delivered at institutes during visits}
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
\quad \quad \quad {$21^{st}$ May 2020} &{\bf University of Utah, School of Computing}{Provable training of depth$-2$ nets.}{}{}{}\\
\quad \quad \quad {$21^{st}$ Jan 2020}&{\textbf{NVIDIA AI Lab, Toronto}}{ Mathematics of training small neural nets and their PAC-Bayesian risk bounds.}{}{}{}\\
\quad \quad \quad {$22^{th}$ Nov 2019}&{\textbf{University of Michigan, Biostatistics}}{ Mathematics of training small neural nets and their PAC-Bayesian risk bounds.}{}{}{}\\
\quad \quad \quad {$13^{th}$ Nov 2019}&{\bf Harvard University, Applied Mathematics}{ Mathematics of training small neural nets and their PAC-Bayesian risk bounds.}{}{}{}\\
\quad \quad \quad {$22^{th}$ Aug 2019}&{\textbf{Google Brain, Mountain View}}{ Mathematics of training small neural nets and their PAC-Bayesian risk bounds. }{\href{https://www.overleaf.com/read/nxxkkmbzvszb}{{\bf \color{violet}[Slides at this link]}}}{}{}\\

\quad \quad \quad {$16^{th}$ Jan 2019}&{\textbf{\bf The Institute of Mathematical Sciences}}{ A $2$ hour long deep-learning survey talk as a part of their graduate course ``Mathematics Of ML". }{\href{https://www.overleaf.com/read/hfchznwmbkwg}{{\bf \color{violet}[Slides at this link]}}}{}{}\\
\end{tabular}
\end{table}

\begin{table}[H]
    \begin{tabular}{r p{12cm}}
\quad \quad \quad {$25^{th}$ July 2018}&{\textbf{Vector Institute For Artificial Intelligence}}{ A $2$ hour long survey talk on our theorems on deep learning. }{\href{https://v2.overleaf.com/read/zyfmrcjfprvr}{{\bf \color{violet}[Slides at this link]}}}{}{}\\

\quad \quad \quad {$14^{th}$ Nov 2017}&{\bf Massachusetts Institute of Technology (MIT), Department of Mathematics}{ A $1$ hour survey talk on our deep net theorems.}{(contents absorbed into the above survey)}{}{}{}\\

\quad \quad \quad {$1^{st}$ Dec 2016}&{\bf Indian Institute of Science Education and Research (IISER), Pune}{ Understanding deep neural networks with ReLU activation.}{}{}{}{}\\

\quad \quad \quad {$28^{th}$ Sep 2015} &{\bf IBM Research Laboratory, Delhi (Bangalore)}{ Can we construct Ramanujan graphs?}{\href{https://www.overleaf.com/read/jkrtxpspqxwh}{{\bf \color{violet}[Slides at this link]}}}{}{}\\

\quad \quad \quad {$2^{nd}$ Sep 2015}&{\bf Johns Hopkins University}{ Possible approaches towards constructing Ramanujan graphs in deterministic polynomial time.}{}{}{}\\

\quad \quad \quad {$2^{nd}$Apr 2015}&{\bf UIUC}{ Sum of squares proof system and hypercontractive inequality for characterizing small-set expansion.}{\href{https://www.overleaf.com/read/bwxdgstmbtgg}{{\bf \color{violet}[Slides at this link]}}}{}{}\\

\quad \quad \quad {Jun 2014}&{\bf Indian Institute of Science (IISc.)}{ Progress on understanding Klebanov's conjecture about Renyi entropy of the criticial $O(N)$-model.}{}{}{}{}
\end{tabular}
\end{table}

\section*{Funding awarded to attend conferences}
\begin{table}[H]
\begin{tabular}{r p{12cm}}
\quad \quad \quad {$29^{th}$ Oct -$2^{nd}$ Nov $2018$} &{ Simons' Institute (Berkeley) workshop on ``Robust and High-Dimensional Statistics",}{ Duncan Fund}{}{}{}\\

\quad \quad \quad {$17^{th}$-$22^{nd}$ June $2018$} &{ IEEE International Symposium on Information Theory (ISIT), 2018}\\ &{Student Travel Award}{}{}{}\\

\quad \quad \quad {$30^{th}$ April-$3^{rd}$ May $2018$}&{ International Conference on Learning Representations (ICLR), 2018}\\&{Student Travel Award}{}{}{}\\

\quad \quad \quad {$22^{nd}$-$23^{rd}$ June $2016$}&{Chaining Methods and their Applications to Computer Science, Harvard University}{ I received funding from NSF (National Science Foundation) to attend this workshop.}{}{}{}\\

\quad \quad \quad {$24^{th}$ June $2016$}&{Theory of Deep Learning, ICML 2016}\\ &{ I received departmental funding to attend this conference.}{}{}{}\\

\quad \quad \quad {$12^{th}$-$15^{th}$ June $2010$} &{I was selected to attended the International Congress of Mathematicians (ICM) satellite meeting on ``Geometric Topology and Riemannian Geometry" at the Indian Institute of Science, Bangalore, India}{}{}{}
\end{tabular}
\end{table}

\section*{Major graduate courses completed in mathematics, computer science and physics}
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
\quad \quad \quad {Mathematics}&{\bf Algebraic Geometry : }{Algebraic curves and Riemann surfaces}{}{}{}{}\\
\quad \quad \quad {}&{\bf Optimization : }{Introduction to Convexity, Sparse Recovery and Compressed Sensing, Nonlinear Optimization II, Machine Learning }{}{}{}{}\\
\quad \quad \quad {}&{\bf Probability : }{Probability Theory I, High dimensional probability and statistical learning theory, Stochastic Calculus}{}{}{}{}\\
\quad \quad \quad {}&{\bf Analysis : }{Introduction to Harmonic Analysis and Its Applications }{}{}{}{}\\
\quad \quad \quad{ Computer Science}&{\bf Theoretical  CS : }{Algorithms, Computational Complexity, Spectral Graph Theory, Advanced Cryptography, Pseudorandomness}{}{}{}\\

\quad \quad \quad{Physics} &{\bf Field Theory : } {Quantum Field Theory , Particle physics, Phase transitions and Critical Phenomenon}{}{}{}
\cventry{}{Gravity} {General Relativity}{}{}{}
\end{tabular}
\end{table}

\section*{Undergraduate awards}
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
\quad \quad \quad{2008}&{\bf Lindau conference,}{ Selected as a member of the Indian contingent to The Nobel Laureate Meetings at Lindau (Physics). I delivered a presentation at the DFG Headquarters in Bonn, Germany on behalf of the Indian contingent}{}{}{}~\\

\quad \quad \quad{2003-2008}&{\bf KVPY,}{ I was among the $40$ students across India who were awarded the Kishore Vaigyanik Protsahan Yojana (KVPY) scholarship,
from the Department of Science and Technology, Govt.  of India. In India at the undergraduate level KVPY scholarship has the highest monetary value.}{}{}{}~\\

\quad \quad \quad{2006}&{\bf CalTech,}{ Selected to the California Institute of Technology as an international transfer student. Selection was through 2 subjective tests in Physics and Mathematics}{}{}{}~\\

\quad \quad \quad{2006}&{\bf SINP,}{ Selected to the ``Undergraduate Associateship" in Physics at the Saha Institute of Theoretical Physics (SINP) which provided me an annual travel and book grant for 2 years}{}{}{}
\end{tabular}
\end{table}

\section*{High-school achievements}
\begin{table}[H]
    \begin{tabular}{r p{12cm}}
\quad \quad \quad{2005}&{\bf ISI,}{ Selected to the prestigious B.Stat program of the Indian Statistical Institute (ISI) through one of the most competitive nationwide mathematics examination consisting of two levels of written testing and an hour long problem solving interview}{}{}{}\\

\quad \quad \quad{2005}&{\bf Presidency College, Kolkata,}{ Secured rank $1$ and $4$ at the undergraduate physics and mathematics entrance tests of the Presidency College, Kolkata.}{}{}{}\\

\quad \quad \quad{2002}&{\bf NSO,}{ Secured All India Rank $35$ in the $4^{th}$ National Science Olympiad (NSO)}{}{}{}{}
\end{tabular}
\end{table}


\begin{table}[H]
    \begin{tabular}{r p{12cm}}
    \end{tabular}
\end{table}

==> Useless/Chapter_Neural_Training.tex <==
\chapter{\vspace{10pt} Provable Training Of Certain Depth $2$ Nets}\label{chaptrain} 

\section{Introduction}

In this section we will prove trainability of classes of depth $2$ neural nets under more general settings than hitherto known till date. Towards identifying the minimal open questions in this field we need to define what we mean by ``training a neural net". Unless particularly specified we shall use this phrase to mean either of the following two mutually exclusive objectives : {\color{blue}  Objective $1$ (Semi-Realizable)} Recover upto some constant error the prameters of the underlying net when the data comes as tuples $(\x,\y)$ with $\y$ being a possibly noisy output of a net when given $\x$ as input. {\color{blue} Objective $2$ (Semi-Agnostic)} Approximative solve ERM or true risk minimization when data comes as tuples $(\x,\y)$ with no obvious functional relationship between $\x$ and $\y$ but there could be geometrical or statistical assumptions about the $\x$ and $\y$. 

We note that its not very interesting to work in the fully agnostic setting as in that case training even a single ReLU gate can be SPN-hard as shown in \cite{goel2016reliably}  On the other hand the simplifications that happen for infinitely large networks have been discussed since \cite{neal1996priors} and this theme has had a recent resurgence in works like \cite{chizat2018global, jacot2018neural}. Eventually this lead to an explosion of literature getting linear time training of various kinds of neural nets when their width is a high degree polynomial in training set size, inverse accuracy and inverse confidence parameters (a very {\it unrealistic} regime),  \cite{lee2018deep, wu2019global,dugradient, su2019learning,kawaguchi2019gradient,huang2019dynamics,allen2019convergenceDNN,allen2019learning,allen2019convergenceRNN,du2018power,zou2018stochastic,zou2019improved,arora2019exact,arora2019harnessing,li2019enhanced,arora2019fine,lee2018deep}. The essential essential proximity of this regime to kernel methods have been thought of separately in \cite{allen2019can,wei2019regularization} 


Even in the wake of this progress, it remains unclear as to how any of this can help establish rigorous guarantees about ``smaller" neural networks or more pertinently of constant size neural nets which is a regime closer to what is implemented in the real world. Thus motivated we can summarize what is open about training depth $2$ nets into the following two questions, 

\begin{enumerate}
    \item {\bf Question $1$} Can {\it any} algorithm train a ReLU gate to $\epsilon-$accuracy in $\poly(\frac 1 \epsilon)$ time using  neither symmetry nor compact support assumptions on the distribution? 
    \begin{itemize}
        \item {\bf Question $1.5$} Can a single ReLU gate be trained using (S) GD with (a) random/arbitrary initialization and (b) weakly constrained distribution (at least non-Gaussian and preferably non-compactly supported) distribution)?
    \end{itemize}
    \item {\bf Question $2$} Can a neural training algorithm work with the following naturally wanted properties being simultaneously true? 
    \begin{enumerate} 
    {\small 
    \item Nets of depth $2$ with a constant/small number of gates. 
    \item The training data instances (and maybe also the noise) would have non-Gaussian non-compactly supported distributions. 
    \item Less structural assumptions on the weight matrices than being of the single filter convolutional type.
    \item $\epsilon-$approximate answers be obtainable in at most $\poly(\frac {1}{\epsilon})$ time.
    }
    \end{enumerate} 
\end{enumerate}

%\newpage 
\subsection{A summary of our results}

We make progress on some of the above fronts by drawing inspiration from two distinct streams of literature and often generalizing and blending techniques from them. First of them are the different avatars of the iterative stochastic non-gradient ``Tron" algorithms analyzed in the past like, \cite{rosenblatt1958perceptron, pal1992multilayer, freund1999large, kakade2011efficient, klivans2017learning, goel2017learning, goel2018learning}. The second kind of historical precedence that we are motivated by are the different works which have shown how some of the desired theorems about gradient descent can be proven if designed noise is injected into the algorithm in judicious ways, \cite{raginsky2017non, xu2018global, 
zhang2017hitting, durmus2019analysis, lee2019online, jin2018local, mou2018generalization, li2019generalization} To the best of our knowledge none of the convergence results among these can be directly lifted to any neural net because these proofs crucially leverage either convexity or very strong smoothness assumptions on the optimization objective.  

Also critical to our work is that we focus on the following class of depth $2$ nets, 

\begin{definition}[{\bf Single Filter Neural Nets Of Depth $2$}]\label{net} 
Given a set of $k$ matrices $\A_i \in \R^{r\times n}$ and an activation function $\sigma : \R \rightarrow \R$ we call the following depth $2$, width $k$ neural net to be a ``single filter neural net" defined by the matrices $\A_1,\ldots,\A_k$
\[
\R^n \ni \x \mapsto f_{\w}(\x) = \frac{1}{k} \sum_{i=1}^k \sigma \Big ( \w^\top \A_i\x \Big ) \in \R 
\]
\end{definition}

Note that the above class of nets includes any single $\relu$ gate for $k=1, \A_1 = I_{n\times n}$ and it also includes any depth $2$ convolutional neural net with a single filter for the $\A_i's$ being such that all of its entries are $0$ except that each row has exactly one $1$ and each column has at most one $1$. 

The results we present here about training single filter neural nets of depth $2$ in the (noisily) realizable setting can be divided into two kinds, 

\subsubsection{Guarantees without the assumption of parity symmetry on the data distribution}

In Section \ref{sec:GDNoiseReLU} we show the first-of-its-kind analysis of gradient descent on a $\relu$ gate albeit when assisted with the injection of certain kinds of noise. We assume that the labels in the data are realizable but we make no assumptions on the distribution of the domain. In this setting previously there have been no results for the $\relu$ gate. We make progress by showing that such a noise assisted GD in such a situation has a ``diffusive" behaviour about the global minima i.e  i.e after {\rm T} steps of the algorithm starting from {\it anywhere}, w.h.p at least one of the steps of the algorithm was within $\sqrt{T}$ distance of the global minima of the function.  %w.h.p it stays within a ball of radius $\sim \sqrt{T}$ about the global minima after $T$ steps of starting from any {\it arbitrary} initial point. 

\remark We would like to emphasize to the reader that in such a distribution free regime as above, there are {\it no} algorithms known yet which can provably train. Also note that the result is parametric in the magnitude of the added noise and hence one can make the algorithm be arbitrarily close to being a pure gradient descent. 

In Section \ref{sec:GLMTron} we re-analyze a known algorithm called ``GLM-Tron" to show that it can do approximate parameter recovery on any Lipschitz gate (in particular a $\relu$ gate) in the noisily realizable setting while no assumptions are being made on the distribution of the noise beyond their boundedness - hence the noise can be {\it ``adversarial"}. We also point out how the result can be improved under some  assumptions on the noise making it more benign. 


\subsubsection{Guarantees with the assumption of parity symmetry on the data distribution} 

In Section \ref{sec:NeuroTronD2FBSingle} we allow ourselves a symmetry assumption on the data to show a generalization of the GLM-Tron algorithm (to what we call the ``Neuro-Tron")  that can provably do approximate parameter recovery for an interesting class of depth $2$ nets with Leaky-$\relu$ activation (in particular with $\relu$ activations). We continue to allow the noise to be adversarial albeit bounded.  This multi-gate form of GLM-Tron turns out to be significantly more mathematically complicated to analyze. 

\remark It is to be noted in the above that in the cases where we leverage parity symmetry of the data distribution, we are also able to write the proof for arbitrary width depth $2$ net of the type we focus on.  


\section{Dynamics of noise assisted gradient descent on a single $\relu$ gate}\label{sec:GDNoiseReLU}

Given the seemingly extreme difficulty with being able to prove convergence with SGD or GD we focus on analyzing a noise assisted version of gradient dynamics on a ReLU gate in the realizable setting as given in Algorithm \ref{GLDReLUParam}. In this setting we will see that we have some non-trivial control while trying to do empirical risk minimization and making no assumptions about the training data beyond realizability.  

\begin{algorithm}[h!]
\caption{Noise Assisted Gradient Dynamics on a single ReLU gate (realizable data)}
\label{GLDReLUParam}
\begin{algorithmic}[1]
\State {\bf Input:} We assume being given a step-length sequence $\{ \eta_t\}_{t=1,2,\ldots}$ %and a conditionally unbiased noisy oracle 
and $\{ (\x_i,y_i) \}_{i=1,\ldots,S}$ tuples where $y_i = f_{\w_*}(\x_i)$ for some $\w_* \in \R^n$ where $f_\w$ is s.t \[ \R^n \ni \x \mapsto  f_\w (\x)= \textrm{ReLU}(\w^\top \x) = \max \{0, \w^\top \x \} \in \R \]
\State Start at $\w_1$ 
%\Comment {\tt {\color{blue} This choice can be made randomly too, like choose $\w_1 \sim {\cal N}(0,I_n)$}}
\For {$t = 1,\ldots$}
    %\State $\x_t \sim {\cal D}$
    %\State The oracle on being queried at $\x_t$ returns $y_t = \text{ReLU}(\w^{*\top} \x_t)$ %where, $\mathbb{E}[\xi_t \mid \x_t] = 0$
    \State Choice of Sub-Gradient $:= \g_t = -\frac{1}{S} \sum_{i = 1}^S \mathbf{1}_{\w_t^\top \x_i \geq 0} \Big (y_i - f_{\w_t}(\x_i) \Big )  \x_i$
    \State $\w_{t+1} := \w_t - \eta_t (\g_t + \xi_{t, 1}) +  \sqrt{\eta_t} \xi_{t, 2}$\Comment {\tt {\color{blue} $\xi_{t, 1}$ is $0$ mean bounded random variable}}
    \State \Comment {\tt {\color{blue} $\xi_{t, 2}$ is a $0$ mean random variable s.t $ \E \Big [ \norm{\xi_{t,2}}^2 \Big ] < d$}}
\EndFor 
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{confine:GLDReLUParam}
 We analyze Algorithm \ref{GLDReLUParam} with constant step length $\eta_t = \eta$ %and when $\xi_{t,1}$ and $\xi_{t,2}$ are uncorrelated random variables for all $t$. 
 Let $C := \max_{i=1,\ldots,S} \norm{\x_i}$, $S_1 >0$ be s.t $\forall t=1,\ldots, \norm{\xi_{t,1}} \leq S_1$ and $\xi_2$ be a random variable defined to have the same distribution as any of the $\{\xi_{t,2}\}_{t=1,\ldots}$

Then for any $i_{\max} \in \Z^+$, $\lambda >0$, $C_L \in (0, \sqrt{d}), i_{\max}(2\eta^2C^4) < 1$ and $r_*^2 \geq \lambda + \norm{\w_0 - \w_*}^2 + i_{\max}\Big \{ 2\eta^2 (C^4 r_*^2 + S_1^2) + \eta d   \Big \}$ we have, 

\begin{align}
    \nonumber &\mathbb{P} \Bigg [  \exists i \in \{ 1,\ldots,i_{\max} \} \mid \norm{\w_i - \w_*} > r_* \Bigg ]\\
    \nonumber &\leq  i_{\max} \Bigg (  \mathbb{P} \Big [ \norm{\xi_2} > C_L \Big ] +  \exp \Bigg \{ - \frac{\lambda^2}{2i_{\max}} \times \frac{1}{2 \sqrt{\eta} C_L \Big ( r_* + \eta (C^2r_* + S_1 ) \Big ) + \eta \Big ( 2S_1r_* + d + 2C^2r_*^2 +  2\eta ( C^4r_*^2 + S_1^2 ) \Big )}  \Bigg \} \Bigg ) 
\end{align}

\end{theorem}

\remark 
Thus for $\eta$ small enough and if $\mathbb{P} \Big [ \norm{\xi_2} > C_L \Big ]$ is small then with significant probability the noise assisted gradient dynamics on a single $\relu$ gate in its first $i_{\max}$ steps remains confined inside a ball around the true parameters of radius, 

\[ r_* \geq \sqrt { \frac{\lambda + \norm{\w_0 - \w_*}^2 + i_{\max}(\eta d + 2\eta^2 S_1^2)}{1 - 2i_{\max} \eta^2C^4} } \]

Larger the $\lambda >0$ we choose more confinement we get in the corresponding larger ball.

\remark From the above argument we can as well remove the $\xi_{2,t}$s and the essential phenomenon will still hold by following the same proof. But we have chosen to keep it with a view towards future applications. 


\note{
Assume $(\xi_2)_{i} \sim {\cal N}(0,\sigma_i)$ for $i = 1, \ldots,d$. For this case we have from Equation 3.5 in the Ledoux-Talagrand book that $\mathbb{P} \Big [ \norm{\xi_2} > C_L \Big ] \leq 4 e^{-\frac{C_L^2}{8 \times \E \Big [ \norm{\xi_2}^2 \Big ]}}$. Then we need, $\exp{-\frac{C_L^2}{8 \times \E \Big[ \norm{\xi_2}^2 \Big ]}} < \frac{1}{4i_{\max}}$. Note that $\E \Big [ \norm{\xi_2}^2 \Big ] = \sum_{i=1}^d \sigma_i^2$ and hence the above condition puts a smallness constraint on the variances of the Gaussian noise depending on how large an $i_{\max}$ we want,  $\sum_{i=1}^d \sigma_i^2 < \frac{C_L^2}{8 \log (4i_{\max})}$.
}


%\newpage 
\begin{proof}[{\bf Proof of Theorem \ref{confine:GLDReLUParam}}]  
~\\
For convenience we will use the notation, $\tilde{\g}_t := \g_t + \xi_{t,1}$ and define $r>0$ s.t $\norm{\w_t - \w_*}\leq r$.

Firstly we want to get a upper-bound on the quantity $\|\w_{t + 1} - \w_*\|^2 - \|\w_{t} - \w_*\|^2$.
\begin{align}
    \nonumber \|\w_{t + 1} - \w_*\|^2 
    &= \|\w_t - \eta_t \tilde \g_t + \sqrt{\eta_t} \xi_{t, 2} - \w_*\|^2\\
    &= \|\w_t - \w_*\|^2 + \|-\eta_t \tilde \g_t + \sqrt{\eta_t} \xi_{t, 2}\|^2 + 2 \langle \w_t - \w_*, -\eta_t \tilde \g_t + \sqrt{\eta_t} \xi_{t, 2}\rangle \label{combine1}
\end{align}

Expanding the second term above as, $\|-\eta_t \tilde \g_t + \sqrt{\eta_t} \xi_{t, 2}\|^2 
    = \eta^2_t \|\tilde \g_t\|^2 + \eta_t \|\xi_{t, 2}\|^2 - 2 \eta_t^{3/2} \langle \tilde \g_t, \xi_{t, 2} \rangle$
    
and combining into \ref{combine1}, we have, 

\begin{align}\label{stepdecrease1}
\nonumber  &\|\w_{t + 1} - \w_*\|^2 - \|\w_t - \w_*\|^2 \\
\nonumber &= \langle \xi_{t, 2}, -2 \eta_t^{3/2} \tilde \g_t + 2 \sqrt{\eta_t} \w_t - 2 \sqrt{\eta_t} \w_* \rangle + \eta_t \|\xi_{t, 2}\|^2 + \eta_t^2 \| \tilde \g_t \|^2 - 2 \eta_t \langle \w_t - \w_*, \tilde \g_t \rangle\\
\nonumber &= \langle \xi_{t, 2}, -2 \eta_t^{3/2} \tilde \g_t + 2 \sqrt{\eta_t} \w_t - 2 \sqrt{\eta_t} \w_* \rangle + \eta_t \|\xi_{t, 2}\|^2 + \eta_t^2 \| \tilde \g_t \|^2 - 2 \eta_t \langle \w_t - \w_*, \xi_{t, 1} \rangle\\
\nonumber &- 2 \eta_t \langle \w_t - \w_*, \g_t \rangle\\
 &\leq -2\eta_t \langle \w_t - \w_* , \xi_{t,1} \rangle + \eta_t^2 \norm{\tilde \g_t}^2 + 2 \sqrt{\eta_t} \langle \xi_{t,2}, -\eta_t \tilde \g_t + \w_t - \w_* \rangle + \eta_t \norm{\xi_{t,2}}^2 
\end{align}

In the last line we have used the Lemma \ref{corr} which shows this critical fact that $\langle \w_t - \w_*, \g_t \rangle \geq 0$. 

Now we use the definition $\tilde \g_t = \g_t + \xi_{t, 1}$ on the 2nd term in the RHS of equation \ref{stepdecrease1} to get, 

\begin{align}\label{stepdecrease2} 
\nonumber &\|\w_{t + 1} - \w_*\|^2 - \|\w_t - \w_*\|^2\\
\nonumber &\leq -2\eta_t \langle \w_t - \w_* , \xi_{t,1} \rangle + 2\eta_t^2 (\norm{\g_t}^2 + \norm{\xi_{t,1}}^2) + 2 \sqrt{\eta_t} \langle \xi_{t,2}, -\eta_t \tilde{\g_t} + \w_t - \w_* \rangle + \eta_t \norm{\xi_{t,2}}^2\\
\nonumber &\leq -2\eta_t \langle \w_t - \w_* , \xi_{t,1} \rangle + 2\eta_t^2 (\norm{\g_t}^2 + S_1 ^2) -  2 \sqrt{\eta_t} \langle \xi_{t,2} , \eta_t \tilde{\g}_t \rangle + 2 \sqrt{\eta_t} \langle \xi_{t,2}, \w_t - \w_* \rangle + \eta_t \norm{\xi_{t,2}}^2\\ 
&\leq 2\eta_t^2 (\norm{\g_t}^2 + S_1 ^2) + \eta_t d  + \Big [  -2\eta_t \langle \w_t - \w_* , \xi_{t,1} \rangle - 2 \sqrt{\eta_t} \langle \xi_{t,2} , \eta_t \tilde{\g}_t \rangle + 2 \sqrt{\eta_t} \langle \xi_{t,2}, \w_t - \w_* \rangle + \eta_t (\norm{\xi_{t,2}}^2 - d) \Big ] 
\end{align}


% Now we recall that $\xi_{t,1}$ and $\xi_{t,2}$ are both $0$ mean random variables and uncorrelated and hence everything inside the $\Big [ \text{ } \Big ]$ is an expectation $0$ random variable conditioned w.r.t the sigma algebra generated by $\w_0,\w_1,\ldots,\w_t$. 


Now we will get a finite bound on $\norm{\g_t}^2$ by invoking the definition of $r$ and $C$ as follows,

\begin{align}\label{gradnorm}
\g_t = \frac{1}{S} \sum_{i = 1}^S \Big (y_i - {\rm ReLU}(\w_t^\top \x_i) \Big ) \mathbf{1}(\w_t^\top \x_i \geq 0) (-\x_i)
\implies \norm{\g_t} \leq \frac{1}{S} \times C \sum_{i=1}^S \vert (\w_* - \w_t) ^\top \x_i \vert \leq C^2r   
\end{align}

Substituting this back into equation \ref{stepdecrease2} we have, 

\begin{align}\label{stepdecrease3}
\nonumber &\|\w_{t + 1} - \w_*\|^2 - \|\w_t - \w_*\|^2\\
\nonumber &\leq \Big \{ 2\eta_t^2 (C^4 r^2 + S_1^2) + \eta_t d   \Big \}\\ 
&+ \Big [  -2\eta_t \langle \w_t - \w_* , \xi_{t,1} \rangle - 2 \sqrt{\eta_t} \langle \xi_{t,2} , \eta_t \tilde{\g}_t \rangle + 2 \sqrt{\eta_t} \langle \xi_{t,2}, \w_t - \w_* \rangle + \eta_t (\norm{\xi_{t,2}}^2 - d) \Big ] 
\end{align}


We define $\w'_0 = \w_0$ and $\xi_{t,2}' = \min \Big \{ C_L, \norm{\xi_{t,2}} \Big \} \frac{\xi_{t,2}}{\norm{\xi_{t,2}}}$ and $C_L \in (0,\sqrt{d})$. 

Now we define a delayed stochastic process associated to the given algorithm, 

\[ \w'_{t+1} = \w'_t \delta_{\norm{\w'_t - \w_*} \geq r} + \Big (\w'_t - \eta_t \tilde{\g}_t + \sqrt{\eta_t}\xi_{t,2}' \Big )\delta_{\norm{\w'_t - \w_*} < r}  \]

Associated to the above we define another stochastic process as follows, 

\[ y_t = \norm{\w_t' - \w_*}^2 - t\Big \{ 2\eta_t^2 (C^4 r^2 + S_1^2) + \eta_t d   \Big \} \] 

Now in Lemma \ref{bounded} we prove the crucial property that for $\eta_t = \eta >0$ a constant, the stochastic process $\{y_t\}_{t=0,1,\ldots}$ is a bounded difference process i.e $\vert y_{t+1} - y_t \vert \leq k$ for all $t=1,\ldots$ and 

\[ k = 2 \sqrt{\eta} C_L \Big ( r + \eta (C^2r + S_1 ) \Big ) + \eta \Big ( 2S_1r + d + 2C^2r^2 +  2\eta ( C^4r^2 + S_1^2 ) \Big ) \] 

Now note that $y_0$ is a constant since $\w_0$ is so. Also in the {\bf Case $1$} above we have $y_{t+1} - y_t <0$ for $\eta_t = \eta >0$. Further note that the random variables $\xi_{t,1}$ and $\xi_{t,2}$ are not measurable in the sigma algebra (say ${\cal F}_t$) generated by $\{ y_0, \ldots, y_t \}$. Hence if in the {\bf Case $2$} above we take a conditional expectation of the RHS of equation \ref{diff01} w.r.t ${\cal F}_t$ then the first two terms will go to $0$ and the last term will give a negative contribution since $\norm{\xi'_{t,2}} \leq C_L$ and $C_L^2 < d$ by definition.

Thus the stochastic process $y_0,\ldots$ satisfies the conditions of the concentration of measure Theorem \ref{AHSM} and thus we get that for any $\lambda >0$ and $t >0$ and $k$ as defined above, 

\[ \mathbb{P} \Big [ y_t - y_0 \geq \lambda \Big ] \leq e^{-\frac{\lambda^2}{2tk}}  \]

And explicitly the above is equivalent to,

\begin{align*}
    &\mathbb{P} \Big [ \norm{\w_t' - \w_*}^2 - t\Big \{ 2\eta^2 (C^4 r^2 + S_1^2) + \eta d   \Big \} - \norm{\w_0 - \w_*}^2 \geq \lambda \Big ] \\ 
    &\leq \exp \Bigg \{ - \frac{\lambda^2}{2t} \times \frac{1}{2 \sqrt{\eta} C_L \Big ( r + \eta (C^2r + S_1 ) \Big ) + \eta \Big ( 2S_1r + d + 2C^2r^2 +  2\eta ( C^4r^2 + S_1^2 ) \Big )}  \Bigg \} 
\end{align*}

Suppose, $r^2 \geq \lambda + \norm{\w_0 - \w_*}^2 + t\Big \{ 2\eta^2 (C^4 r^2 + S_1^2) + \eta d   \Big \}$ then it follows that,

\begin{align}\label{escape1}
    \nonumber &\mathbb{P} \Big [ \norm{\w_t' - \w_*}^2 \geq r^2 \Big ] \\
    &\leq \exp \Bigg \{ - \frac{\lambda^2}{2t} \times \frac{1}{2 \sqrt{\eta} C_L \Big ( r + \eta (C^2r + S_1 ) \Big ) + \eta \Big ( 2S_1r + d + 2C^2r^2 +  2\eta ( C^4r^2 + S_1^2 ) \Big )}  \Bigg \} 
\end{align}

For the given positive integer $i_{\max}$ consider the event, $E := \Big \{ \exists i \in \{ 1,\ldots,i_{\max} \} \mid \norm{\w_i - \w_*} > r \Big \}$.

Now note that the primed and the unprimed sequences evolve the same way at any time instant unless either (a) $\w'_t$ leaves the $r$ ball of $\w_*$ or (b) the following event $E_t := \{ \norm{\xi_{t,2}} > C_L \}$ happens.  Thus if $E_t$ never happens then the two processes evolve the same. Thus the sample space can be written as a disjoint union of events $A := \cup_{t=1}^{i_{\max}} E_t$ and $B := \cap_{t=1}^{i_{\max}} E_t^c$. 

Let $L_t$ be the event that $t$ is the first time instant when $\w_t$ leaves the ball. Let $L'_t$ be the event that $t$ is the first time instant when $\w'_t$ leaves the ball. And we have argued above that when $B$ happens the two sequences evolve the same which in turn implies $B \cap L_t = B \cap L'_t$.  

Thus we have, $\mathbb{P} \Big [ L_t \Big ] =  \mathbb{P} \Big [ L_t \cap A \Big ] +  \mathbb{P} \Big [ L_t \cap B \Big ] = \mathbb{P} \Big [ L_t \cap A \Big ] +  \mathbb{P} \Big [ L'_t \cap B \Big ]$

And combining with the definition of $E$ we have, 
\[ \mathbb{P} \Big [  E  \Big ] = \sum_{t=1}^{i_{\max}} \mathbb{P} \Big [ L_t \Big ] = \sum_{t=1}^{i_{\max}} \mathbb{P} \Big [ L_t \cap A \Big ] +  \mathbb{P} \Big [ L'_t \cap B \Big ] \leq \mathbb{P} \Big [ A \Big ] +  \sum_{t=1}^{i_{\max}} \mathbb{P} \Big [ L'_t \Big ] \leq \sum_{t=1}^{i_{\max}} \Big ( \mathbb{P} \Big [ E_t \Big ] + \mathbb{P} \Big [ L'_t \Big ] \Big ) \] 

The second equality above is true because $L_t$ are disjoint events.  

We further note that, $\mathbb{P} \Big [ L'_t \Big ] \leq \mathbb{P} \Big [ \norm{\w'_t - \w_*} > r \Big ]$

Hence combining we have,  

\[ \mathbb{P} \Bigg [  \exists i \in \{ 1,\ldots,i_{\max} \} \mid \norm{\w_i - \w_*} > r \Bigg ] \leq \sum_{t=1}^{i_{\max}} \Big ( \mathbb{P} \Big [ \norm{\xi_{t,2}} > C_L \Big ] +  \mathbb{P} \Big [ \norm{\w'_t - \w_*} > r \Big ] \Big ) \] 

We recall (a) the definition of the random variable $\xi_2$ and (b) the assumption that $r_*^2 \geq \lambda + \norm{\w_0 - \w_*}^2 + i_{\max}\Big \{ 2\eta^2 (C^4 r_*^2 + S_1^2) + \eta d   \Big \}$ and thus invoking equation \ref{escape1} on each of the summands in the RHS above (with $r=r_*$) we can infer that, 

\begin{align}
    \nonumber &\mathbb{P} \Bigg [  \exists i \in \{ 1,\ldots,i_{\max} \} \mid \norm{\w_i - \w_*} > r_* \Bigg ]\\
    \nonumber &\leq  i_{\max} \Bigg (  \mathbb{P} \Big [ \norm{\xi_2} > C_L \Big ] +  \exp \Bigg \{ - \frac{\lambda^2}{2i_{\max}} \times \frac{1}{2 \sqrt{\eta} C_L \Big ( r_* + \eta (C^2r_* + S_1 ) \Big ) + \eta \Big ( 2S_1r_* + d + 2C^2r_*^2 +  2\eta ( C^4r_*^2 + S_1^2 ) \Big )}  \Bigg \} \Bigg ) 
\end{align}

This proves the theorem we wanted.
\end{proof} 

%\newpage 
\begin{lemma}\label{corr}
$\langle \w_t - \w_*, \g_t \rangle \geq 0$
\end{lemma}
\begin{proof} 
We can obtain a (positive) lower bound on the inner product term $\langle \w_t - \w_*, \g_t \rangle$, 
\begin{align*}
    &\langle \w_t - \w_*, \g_t \rangle \\
    &= -\frac{1}{S} \sum_{i = 1}^S \Big \langle \w_t - \w_*, \Big(y_i - {\rm ReLU}(\w_t^\top \x_i) \Big) \mathbf{1}(\w_t^\top \x_i \geq 0) \x_i \Big \rangle\\
    &= -\frac{1}{S} \sum_{i = 1}^S \Big (\w_t^\top \x_i - \w^{*\top}\x_i \Big) \Big({\rm ReLU}(\w^{*\top}\x_i) - {\rm ReLU}(\w_t^\top \x_i) \Big) \mathbf{1}(\w_t^\top \x_i \geq 0)\\
    &= \frac{1}{S} \sum_{i = 1}^S \Big (\w^{*\top}\x_i - \w_t^\top \x_i \Big) \Big({\rm ReLU}(\w^{*\top}\x_i) - {\rm ReLU}(\w_t^\top \x_i) \Big) \mathbf{1}(\w_t^\top \x_i \geq 0)\\
    &\geq \frac{1}{S} \sum_{i = 1}^S \Big({\rm ReLU}(\w^{*\top}\x_i) - {\rm ReLU}(\w_t^\top \x_i) \Big)^2 \mathbf{1}(\w_t^\top \x_i \geq 0) \\
    %\quad \text{as $(a - b) \geq {\rm ReLU(a) - \}
\end{align*}
\end{proof} 


\begin{lemma}\label{bounded} 
If for all $t=0,\ldots$ we have $\eta_t = \eta$ a constant $>0$ then the stochastic process $\{y_t\}_{t=0,1,\ldots}$ is a bounded difference stochastic process i.e there exists a constant $k >0$ s.t for all $t=1,\ldots$, $\vert y_{t+1} - y_t \vert \leq k$
\end{lemma}

\begin{proof}
We have 2 cases to consider. 

\paragraph{Case 1 : $\norm{\w_t' - \w_*} \geq r$}
~\\
\begin{align}\label{noshift}
y_{t+1} - y_t &= -(t+1)(2\eta_{t+1}^2(C^4r^2 + S_1^2 )+\eta_{t+1}d) + t(2\eta_t^2(C^4r^2 + S_1^2) + \eta_t d)\\
 &= 2(C^4r^2 + S_1^2) \Big \{ t \eta_t^2 - (t+1)\eta_{t+1}^2 \} + d \Big \{ t\eta_t - (t+1)\eta_{t+1}\Big \} \nonumber
\end{align}

%\note{Constant step length helps!?}

\paragraph{Case 2 : $\norm{\w_t' - \w_*} < r$}
~\\
Repeating the calculations as used to get equation \ref{stepdecrease3} but with $\xi'_{t,2}$ instead of $\xi_{t,2}$ we will get,  
\begin{align}\label{diff01}
    y_{t+1} - y_t &\leq -2\eta_t \langle \w_t - \w_* , \xi_{t,1} \rangle - 2 \sqrt{\eta_t} \langle \xi'_{t,2} , \eta_t \tilde{\g}_t \rangle + 2 \sqrt{\eta_t} \langle \xi_{t,2}', \w_t - \w_* \rangle + \eta_t (\norm{\xi_{t,2}'}^2 - d)
\end{align}

And by Cauchy-Schwartz the above implies,  
\begin{align}\label{diff1}    
    y_{t+1} - y_t \leq 2\eta_tS_1r + 2\sqrt{\eta_t}(r + \eta_t (C^2r + S_1) )C_L + \eta_t (C_L^2 - d)
\end{align}

Further repeating the calculations as used to get equation \ref{stepdecrease3} but with $\xi'_{t,2}$ instead of $\xi_{t,2}$ we will get,  

\begin{align*}
\| \w'_t - \w_*\|^2 - \|\w'_{t + 1} - \w_*\|^2 &\leq 2\eta_t r (\norm{\g_t} + \norm{\xi_{t,1}} ) + 2\sqrt{\eta_t} \Big \langle \xi'_{t,2}  , - \eta_t \tilde{\g}_t + (\w_t - \w_*)  \Big \rangle 
\end{align*}

In the above we invoke the definition of $S_1$ and equation \ref{gradnorm} to get, 

\begin{align}
    \nonumber \|\w'_t - \w_*\|^2 - \|\w'_{t + 1} - \w_*\|^2 &\leq 2\eta_t r (C^2r + S_1 ) + 2\sqrt{\eta_t} \Big \langle \xi'_{t,2}  , - \eta_t \tilde{\g}_t + (\w_t - \w_*)  \Big \rangle \\
    \nonumber &\leq 2\eta_t r (C^2r + S_1 ) + 2\sqrt{\eta_t} C_L (\eta_t (C^2r + S_1) + r  )
\end{align}

Hence we have,

\begin{align}\label{diff2}
    y_t - y_{t+1} &\leq 2\eta_t^2 (C^4 r^2 + S_1^2) + \eta_t d  + 2\eta_t r (C^2r + S_1 ) + 2\sqrt{\eta_t} C_L (\eta_t (C^2r + S_1) + r  )
\end{align}

Combining equations \ref{diff1} and \ref{diff2} we have,  

\begin{align}
    \nonumber \vert y_t - y_{t+1} \vert &\leq 2 \eta_t S_1 r + 2 \sqrt{\eta_t} C_L \Big ( r + \eta_t (C^2r + S_1 ) \Big )\\
     &+ \max \Big \{ \eta_t (C_L^2 - d), \eta_t \Big [ (d + 2C^2r^2) + 2\eta_t ( C^4r^2 + S_1^2 )\Big ]  \Big \} 
\end{align}


If we now invoke the that $\eta_t = \eta$, a positive constant then the above and the previous equation \ref{noshift} can be combined to get for all $t=0,\ldots$, 

\begin{align}
    \nonumber \vert y_t - y_{t+1} \vert &\leq \max \Bigg \{ d \eta + 2(C^4r^2 + S_1^2) \eta^2 \\
\nonumber     &, 2 \eta S_1 r + 2 \sqrt{\eta} C_L \Big ( r + \eta (C^2r + S_1 ) \Big ) + \max \Big \{ \eta (C_L^2 - d), \eta \Big [ (d + 2C^2r^2) + 2\eta ( C^4r^2 + S_1^2 )\Big ]  \Big \} \Bigg \}\\ 
\nonumber     &\leq \max \Bigg \{ d \eta + 2(C^4r^2 + S_1^2) \eta^2 \\
\nonumber     &, 2 \sqrt{\eta} C_L \Big ( r + \eta (C^2r + S_1 ) \Big ) + \eta \Big ( 2S_1r + d + 2C^2r^2 +  2\eta ( C^4r^2 + S_1^2 ) \Big )  \Bigg \}\\
    &\leq  2 \sqrt{\eta} C_L \Big ( r + \eta (C^2r + S_1 ) \Big ) + \eta \Big ( 2S_1r + d + 2C^2r^2 +  2\eta ( C^4r^2 + S_1^2 ) \Big ) 
\end{align}

In the second inequality above we are using the fact that $C_L^2 < d$ as per our previously made choice.  
And this proves the boundedness of the stochastic process $\{y_t\}$ as we set out to prove and a candidate $k$ is the RHS above. 
\end{proof}


\section{GLM-Tron converges on any Lipschitz gate with no symmetry assumption on the data}\label{sec:GLMTron}


\begin{algorithm}[H]
\caption{GLM-Tron (\cite{kakade2011efficient}) }
\label{GLMTron} 
%\label{pac-compare-1}
\begin{algorithmic}[1]
\State {\bf Input:} $\{ (\x_i,y_i) \}_{i=1,\ldots,m}$ and an ``activation function"  $\sigma : \R \rightarrow \R$
%\in \B^d \times [0,1] \}_{i=1,\ldots,m}$ where $(\x,y) \sim {\cal D}$ s.t $\E [ \y \mid \x ] = u (\langle \w, \x \rangle)$,  $\norm{\w} \leq W$ and $\u$ is a non-decreasing $1-$Lipschitz function.
\State $\w_1 =0$
\For {$t = 1,\ldots$}
    %\Comment $h_t(\x) := \sigma \Big ( \langle \w_t , \x\rangle \Big )$
    \State $\w_{t+1} := \w_t + \frac {1}{m} \sum_{i=1}^m \Big ( y_i - \sigma(\langle \w_t , \x_i\rangle) \Big)\x_i$ \Comment {\rm Define} $h_t(\x) := \sigma \Big ( \langle \w_t , \x\rangle \Big )$
\EndFor 
\end{algorithmic}
\end{algorithm}

First we state the following crucial lemma, 

\begin{lemma}\label{stepdecrease} 
Assume that for all $i = 1,\ldots,S$ $\norm{\x_i} \leq 1$ and in Algorithm \ref{GLMTron}, $\sigma$ is a $L-$Lipschitz non-decreasing function. Suppose $\exists \w$ s.t at iteration $t$, we have $\norm{\w_t - \w} \leq W$ and define $\eta >0$ s.t $\norm{\frac {1}{S} \sum_{i=1}^S \Big ( y_i - \sigma (\langle \w, \x_i \rangle) \Big ) \x_i} \leq \eta $. Then it follows that $\forall t = 1,2,\ldots$, 

\[  \norm{\w_{t+1} - \w}^2 \leq \norm{\w_t - \w}^2 -  \Big ( \frac {2}{L} - 1 \Big ) \tilde{L}_S(h_t) + \Big (\eta^2 + 2\eta W(L + 1) \Big ) \]

where we have defined, $\tilde{L}_S(h_t) := \frac {1}{S} \sum_{i=1}^S \Big (h_t(x_i) - \sigma (\langle  \w , \x_i\rangle) \Big)^2 = \frac {1}{S} \sum_{i=1}^S \Big ( \sigma (\langle \w_t, x_i\rangle ) - \sigma (\langle  \w , \x_i\rangle) \Big)^2$
\qed 
\end{lemma}

We give the proof of the above Lemma in Appendix \ref{app:glmtronstep}. Now we will see in the following theorem and its proof as to how the above lemma leads to convergence of the ``effective-ERM", $\tilde{L}_S$ by GLM-Tron on a single gate. 

\begin{theorem}\label{GLMTronReLU} [{\bf GLM-Tron (Algorithm \ref{GLMTron}) solves the effective-ERM on a ReLU gate upto noise bound with minimal distributional assumptions}]
Assume that for all $i = 1,\ldots,S$ $\norm{\x_i} \leq 1$ and the label of the $i^{th}$ data point $y_i$ is generated as, $y_i = \sigma (\langle \w_*, \x_i \rangle ) + \xi_i$ s.t $\forall i, \vert \xi_i \vert \leq \theta$ for some $\theta >0$ and $\w_* \in \R^n$.  If $\sigma$ is a $L-$Lipschitz non-decreasing function for $L < 2$ then in at most $T = \frac {\norm{\w_*}}{\epsilon}$ GLM-Tron steps we would attain parameter value $\w_T$ s.t,  

\[ \tilde{L}_S(h_T) =  \frac {1}{S} \sum_{i=1}^S \Big ( \sigma(\langle \w_T, x_i\rangle ) - \sigma (\langle  \w_* , \x_i\rangle) \Big)^2 < \frac{L}{2-L} \Big ( \epsilon +  (\theta^2 + 2\theta W(L + 1) ) \Big ) \]
\qed 
\end{theorem}

\remark Note that in the realizable setting i.e when $\theta =0$, the above theorem is giving an upperbound on the number of steps needed to solve the ERM on say a $\relu$ gate to $O(\epsilon)$.

\remark We also note that the above theorem does not force any distributional assumption on the $\xi_i$ beyond the assumption of its boundedness. Thus the noise could as well be chosen ``adversarially" upto the constraint on its norm.  

\begin{proof}[Proof of Theorem \ref{GLMTronReLU}]
The equation defining the labels in the data-set i.e $y_i = \sigma (\langle \w_*, \x_i \rangle ) + \xi_i$ with $\vert \xi_i \vert \leq \theta$ along with our assumption that, $\norm{\x_i} \leq 1$ implies that , $\norm{\frac {1}{S} \sum_{i=1}^S \Big ( y_i - \sigma (\langle \w_*, \x_i \rangle) \Big )\x_i} \leq \theta$. Thus we can invoke the above Lemma \ref{stepdecrease} between the $t^{th}$ and the $t+1^{th}$ iterate with $\eta = \theta$ and $W$ as defined there to get,   

\[  \norm{\w_{t+1} - \w_*}^2 \leq \norm{\w_t - \w_*}^2 - \left [   \Big ( \frac {2}{L} - 1 \Big ) \tilde{L}_S(h_t) - (\theta^2 + 2\theta W(L + 1) ) \right ] \]

If $\tilde{L}_S(h_t) \geq \frac{L}{2-L} \Big ( \epsilon +  (\theta^2 + 2\theta W(L + 1) ) \Big )$  then, $\norm{\w_{t+1} - \w}^2 \leq \norm{\w_t - \w}^2 - \epsilon$.  
Thus if the above lowerbound on $\tilde{L}_s(h_t)$ holds in the $t^{th}$ step then at the start of the $(t+1)^{th}$ step we still satisfy, $\norm{\w_{t+1}- \w} \leq W$. Since the iterations start with $\w_1=0$, in the first step we can choose $W = \norm{\w_*}$. Thus in at most $\frac{\norm{\w}}{\epsilon}$ steps of the above kind we can have a decrease in distance of the iterate to $\w$.   

Thus in at most $T = \frac {\norm{\w}}{\epsilon}$ steps we have attained, 

\[ \tilde{L}_S(h_T) = \frac {1}{S} \sum_{i=1}^S \Big ( \sigma (\langle \w_T, x_i\rangle ) - \sigma (\langle  \w_* , \x_i\rangle) \Big)^2 < \frac{L}{2-L} \Big ( \epsilon +  (\theta^2 + 2\theta W(L + 1) ) \Big ) \]

And that proves the theorem we wanted.   
\end{proof}


\begin{theorem}[{\bf Performance guarantees on the GLM-Tron (Algorithm \ref{GLMTron}) in solving the ERM problem with data labels being output of a $\relu$ gate corrupted by benign noise}]\label{GLMTronReLUNoise}
Assume that the noise random variables $\xi_i, i = 1,\ldots,S$ are identically distributed as a centered random variable say $\xi$. Then for $T = \frac{\norm{\w}}{\epsilon}$, we have the following guarantee on the (true) empirical risk after $T$ iterations of GLM-Tron (say $\tilde{L}_S(h_T)$), 

\[ \mathbb{E}_{\{ (\x_i , \xi_i)\}_{i=1,\ldots S}} \Big [ L_S(h_T) \Big ] \leq \E_{\xi} [\xi^2] + \frac{L}{2-L} \Big ( \epsilon +  (\theta^2 + 2\theta W(L + 1) ) \Big ) \]  
\qed 
\end{theorem}


\begin{corollary}
Suppose that instead of assuming $\forall i = 1,\ldots,S$ $\vert \xi_i \vert \leq \theta$ we instead assume that the joint distribution of $\{ \xi_i \}_{i=1,\ldots,S}$ is s.t \[ \mathbb{P} \Big [ \vert \xi_i \vert \leq \theta ~\forall i \in \{1,\ldots,S \} \Big ] \geq 1 - \delta \] Then it would follow that the guarantee of the above Theorem \ref{GLMTronReLUNoise} still holds but now with probability $1-\delta$ over the noise distribution.  
\end{corollary}




\begin{proof}[Proof of Theorem \ref{GLMTronReLUNoise}]
Let the true empirical risk at the $T^{th}-$iterate be defined as, 

\[ L_S(h_T) = \frac {1}{S} \sum_{i=1}^S \Big (\sigma(\langle \w_T, x_i\rangle ) - \sigma (\langle  \w_* , \x_i\rangle) - \xi_i \Big )^2 \] 

Then it follows that,  

\begin{align*}
    &\tilde{L}_S(h_T) - L_S(h_T) = \frac {1}{S} \sum_{i=1}^S \Big ( \sigma (\langle \w_T, x_i\rangle ) - \sigma (\langle  \w_* , \x_i\rangle) \Big )^2 - \frac {1}{S} \sum_{i=1}^S \Big ( \sigma (\langle \w_T, x_i\rangle ) - \sigma(\langle  \w_* , \x_i\rangle) - \xi_i \Big)^2\\
    =& \frac {1}{S} \sum_{i=1}^S \xi_i \Big ( -\xi_i + 2 \sigma (\langle \w_T, x_i\rangle ) - 2 \sigma (\langle  \w_* , \x_i\rangle) \Big )
    = -\frac {1}{S} \sum_{i=1}^S \xi_i^2 +  \frac {2}{S} \sum_{i=1}^S \xi_i \Big ( \sigma (\langle \w_T, x_i\rangle ) - \sigma (\langle  \w_* , \x_i\rangle) \Big )
\end{align*}

By the assumption of $\xi_i$ being an unbiased noise the second term vanishes when we compute, $\mathbb{E}_{\{ (\x_i , \xi_i)\}_{i=1,\ldots S}} \Big [ \tilde{L}_S(h_T) - L_S(h_T) \Big ]$ Thus we are led to,
\[ \mathbb{E}_{\{ (\x_i , \xi_i)\}_{i=1,\ldots S}} \Big [ \tilde{L}_S(h_T) - L_S(h_T) \Big ] = -\frac {1}{m}  \mathbb{E}_{\{ \xi_i\}_{i=1,\ldots S}} \Big [ \sum_{i=1}^m \xi_i^2 \Big ] = -\frac{1}{m} \sum_{i=1}^m \mathbb{E}_{\{ \xi_i\}} \Big [ \xi_i^2 \Big ] = - \E_{\xi} [\xi^2] \] 

For $T = \frac{\norm{\w}}{\epsilon}$, we invoke the upperbound on $\tilde{L}_S(h_T)$ from the previous theorem and we can combine it with the above to say, 

\[ \mathbb{E}_{\{ (\x_i , \xi_i)\}_{i=1,\ldots S}} \Big [ L_S(h_T) \Big ] \leq \E_{\xi} [\xi^2] + \frac{L}{2-L} \Big ( \epsilon +  (\theta^2 + 2\theta W(L + 1) ) \Big ) \] 

This proves the theorem we wanted.  
\end{proof}

In the next section \ref{sec:NeuroTronD2FBSingle} we will see a multi-gate generalization of the above theorem with the added assumption of symmetry in the data and the activation $\sigma$ being constrained to be of the form of a {\rm Leaky-$\relu$}. {\it We will see that the multi-gate version of the above analysis leads to a much more complicated dynamical system to be analyzed.}


\section{Neuro-Tron (multi-gate, depth $2$, single filter, ERM with full-batch, with parity symmetric data)}\label{sec:NeuroTronD2FBSingle}

\begin{algorithm}[H]
\caption{Neuro-Tron (multi-gate, depth $2$, single filter, ERM with full-batch, with parity symmetric data)}
\label{NeuroTronD2FBSingle}
\begin{algorithmic}[1]
\State {\bf Input:} {A training set $T$ of $S$ samples of the form, $\{ (\x_i,y_i)\}_{i=1,\ldots,S}$ where $y_i = \xi_i + f_{\w^*}(\x_i)$ and $f_{\w} : \R^n \rightarrow \R$ a depth $2$ net parameterized by a single ``filter", $\w \in \R^r$}. 
\State {\bf Input :} { A matrix $\M \in \R^{r \times n}$ and a step-length $\eta$. }
\State Start at $\w_1$ 
\For {$t = 1,\ldots$}
    %\State $h_t := f_{\w_t}$
    \State { $\g_t := \mathbf{M} \Big ( \frac{2}{w S} \sum_{i=1}^S \underbrace{\Big (y_i - f_{\w_t}(\x_i) \Big )}_{\text{Current prediction error on the }i^{th}\text{ data}}  \x_i \Big ) $} \Comment{Define $h_t := f_{\w_t}$} 
    \State $\w_{t+1} := \w_t + \eta \g_t$
\EndFor 
\end{algorithmic}
\end{algorithm}

\begin{lemma}\label{NeuroTronD2FBSinglestepdecrease}
Assume that that training set $T := \{ (\x_i,y_i) \mid i=1,\ldots,S \}$ is such that the set $T_\x := \{ \x_i \mid i=1,\ldots,S \}$ is invariant under replacing of each $\x_i$ with $-\x_i$. Further suppose, $\sigma : \R \rightarrow \R$ is mapping, $x \mapsto x\mathbf{1}_{x\geq 0} + \alpha x\mathbf{1}_{x\leq 0}$ for some $\alpha >0$ and $f_{\w} : \R^n \rightarrow \R$ is a neural net which maps as $\x \mapsto \frac{1}{w}\sum_{i=1}^w \sigma \Big (  \langle \A_i^\top \w , \x \rangle \Big )$ for some matrices, $\{\A_i \in \R^{r \times n} \mid {i=1,\ldots,w} \}$ (unknown to the algorithm) and some $\w \in \R^r$ 


Suppose $\beta$ is s.t $T$ and $\w$ satisfy $ \norm{\M \Big ( \frac {1}{S} \sum_{i=1}^S (y_i - f_{\w}(\x_i)) \x_i \Big )} \leq \beta  $. and define ${\rm B} = \max_i \norm{\x_i}$ Then at iteration $t$ of the Algorithm \ref{NeuroTronD2FBSingle}, we will have, 

\begin{align*}
    \nonumber &\norm{\w_{t+1} - \w}^2\\
    \nonumber \leq &\norm{\w_t - \w}^2  - 4\frac{ \eta (1+\alpha)}{2S}  \Big [ (\w - \w_t)^\top \Big ( \bar{\A} \tilde{\Sigma}  \M^\top \Big )  (\w - \w_t) \Big ] \\
    &+4\frac{\eta \beta \norm{\w-\w_t}}{w}\\
    &+ \Big ( \frac{2\eta}{w} \Big )^2 \Bigg ( \beta^2 +  \frac{2\beta{\rm B}^2 L}{w} \times \norm{\w - \w_t}  \sqrt{\lambda_{\max} \Big ( \M^\top \M \Big )} \Big ( \sum_{i=1}^w \sqrt{\lambda_{\max} \Big ( \A_i \A_i^\top \Big )} \Big )  + {\rm B}^2 \lambda_{\max} \Big ( \M^\top \M \Big )  \tilde{L}_S(h_t) \Bigg )
\end{align*}

where, $\tilde{L}_S(h_t) := \frac{1}{S}\sum_{i=1}^S \Big (f_{\w}(\x_i) - f_{\w_t} (\x_i) \Big )^2$, $\tilde{\Sigma} := \Big [ \sum_{i=1}^S  \x_i \x_i^\top \Big ]$ and $\bar{\A} = \frac{1}{w} \sum_{j=1}^w \A_j$
\qed 
\end{lemma}

We prove the above in Appendix \ref{app : NeuroTronD2FBSinglestepdecrease} We note that compared to the single gate situation in the previous section the above dynamical system is significantly more challenging - because now there is no obvious way to say that a large value of $\tilde{L}_S$ will necessarily cause progress towards the global minimum. The absence of this direct argument makes the multi-gate analogue significantly more interesting to analyze despite the use of the specific structure of the activation. 

Also note in the above recursion the appearance of terms linear in ``$\beta \norm{\w - \w_t}$". This is a very unique complication of this case we consider here which we will see in the following theorem to be the crucial term that keeps track of the fact that we make no assumptions about the noise in the labels apart from assuming their boundedness. %{\it In the next section when we write a stochastic form of this algorithm we will make assumptions about the noise distribution being benign in certain ways and that will end up removing these linear terms and thus help the analysis become simpler.} 

In the following theorem and its proof we will see as to how in the realizable setting the above lemma leads to approximate recovery of the ground truth parameters by Algorithm \ref{NeuroTronD2FBSingle}.

\remark Note that there is no relationship enforced by-hand between the label associated with $\x_i$ and the label associated to $-\x_i$.

\begin{definition}
Given the definition of $\tilde{\Sigma}$ as above and a matrix $\M$ of appropriate dimensions, we define the following class of neural functions, 

\[ {\cal N}_{\mathbf{M},\tilde{\Sigma},w} = \Big \{ \R^n \ni \y \mapsto  \frac{1}{w}\sum_{k=1}^w \sigma \Big (  \langle \A_k^\top \w^* , \y \rangle \Big )  \in \R  \mid \bar{\A}\tilde{\Sigma}\mathbf{M}^\top \text{ is PD } \Big \} \]
\end{definition}

\remark If $r \leq n$, $\bar{\A}\tilde{\Sigma}$ is full rank i.e rank $r$ then in the above we can always choosen $\M = \bar{\A}\tilde{\Sigma}$. 

\begin{theorem}\label{NeuroTronD2FBSingleERM} [{\bf Neuro-Tron (multi-gate, depth $2$, single filter, ERM with full-batch, with parity symmetric data) (Algorithm \ref{NeuroTronD2FBSingle}) can do parameter recovery on a class of constant sized depth $2$ nets with minimal distributional assumptions}] Suppose that the data set $T$ and the activation function $\sigma$ are as given in Lemma \ref{NeuroTronD2FBSinglestepdecrease} Further assume that the label of the $i^{th}$ data point $(\x_i, y_i)$ is generated as, $y_i  =  f_{\w^*}(\x_i)$ s.t $f_{\w^*} \in {\cal N}_{\mathbf{M},\tilde{\Sigma},w}$ 

%s.t $\forall i, ~\vert \xi_i \vert \leq \theta$ for some $\theta >0$ and 

If $0 < \lambda_{\min} := \lambda_{\min}(\bar{\A}\tilde{\Sigma}\M^\top)$. Then for $T = O(\log (\frac 1 \epsilon))$ time we would have, $\norm{\w_T - \w^*} \leq \epsilon$ if the samples satisfy the following condition, 

\begin{align}\label{cond1}
       \frac{S^2B^4}{\lambda_{\min}^2} > \frac{(1+\alpha)^2 w^3}{\lambda_{\max} \Big (\M^\top \M \Big ) \lambda_{\max} \Big ( \sum_{j=1}^w \A_j^\top \A_j \Big ) } 
\end{align}
    
% . Then we can get the following kinds of convergences,

% \begin{itemize}
%     \item For $\theta =0$, in $T = O(\log (\frac 1 \epsilon))$ time we would have, $\norm{\w_T - \w^*} \leq \epsilon$ if the samples satisfy the following condition, 
    
%     \begin{align}\label{cond1}
%         \frac{S^2B^4}{\lambda_{\min}^2} > \frac{(1+\alpha)^2 w^3}{\lambda_{\max} \Big (\M^\top \M \Big ) \lambda_{\max} \Big ( \sum_{j=1}^w \A_j^\top \A_j \Big ) } 
%     \end{align}
% \end{itemize}

\qed 
\end{theorem}

%\remark As mentioned earlier note that we make no assumptions about the noise being benign in anyway apart from it being bounded in norm by $\theta$. Hence in the above we can accommodate a bounded ``adversarial noise" too whereby the injected disturbance is somehow carefully crafted as a function of the data point to which it is being added.  


For intuition it might be helpful to note the following special case of the above where the neural net class being trained can be defined in a data-independent way, 

\begin{corollary}
Consider the following class of depth $2$ neural nets, 
\[ {\cal N}_{\mathbf{M},w} = \Big \{ \R^n \ni \y \mapsto  \frac{1}{w}\sum_{k=1}^w \sigma \Big (  \langle \A_k^\top \w^* , \y \rangle \Big )  \in \R  \mid \bar{\A} = \mathbf{M} \Big \} \]
If $\M$ is full-rank and $\tilde{\Sigma}$ is PD, then the above convergence theorem holds as long as $f_{\w^*} \in {\cal N}_{\mathbf{M},w} $
\end{corollary}


\begin{proof}[Proof of Theorem \ref{NeuroTronD2FBSingleERM} ]
With an eye towards future uses we will derive the effective dynamical system in the more general case of the labels being noisily realizable i.e assume that the label of the $i^{th}$ data point $(\x_i, y_i)$ is generated as, $y_i  = \xi_i + f_{\w^*}(\x_i)$ s.t $\forall i, ~\vert \xi_i \vert \leq \theta$ for some $\theta \geq 0$ 

Hence we have that $\norm{\frac {1}{S} \sum_{i=1}^S (y_i - f_{\w^*}(\x_i)) \M \x_i} \leq \norm{\frac {1}{S} \sum_{i=1}^S \xi_i \M \x_i} \leq \frac{\theta}{S} \sum_{i=1}^S \norm{\M \x_i} = B\theta \sqrt{\lambda_{\max} ( \M^\top \M) } $
Thus we can invoke the above Lemma \ref{NeuroTronD2FBSinglestepdecrease} between the $t^{th}$ and the $t+1^{th}$ iterate with $\beta = B\theta \sqrt{\lambda_{\max} ( \M^\top \M) }$ and $\w = \w^*$ and invoke the definition of $\lambda_{\min}$ to get,   

\begin{align}\label{prefinal}
    \nonumber \norm{\w_{t+1} - \w^*}^2 \leq &\norm{\w_t - \w^*}^2  - 4\frac{ \eta (1+\alpha)\lambda_{\min}}{2S} \norm{\w_t - \w}^2 \\
    \nonumber &+4\frac{\eta  \norm{\w_t-\w^*}}{w} \times B\theta \sqrt{\lambda_{\max} ( \M^\top \M) }\\
    \nonumber &+ \Big ( \frac{2\eta B}{w} \Big )^2 \lambda_{\max} \Big ( \M^\top \M \Big ) \Bigg (  \theta^2   +  \frac{2{\rm B} L \theta }{w} \times \norm{\w_t - \w^*}   \Big ( \sum_{i=1}^w \sqrt{\lambda_{\max} \Big ( \A_i \A_i^\top \Big )} \Big ) \Bigg ) \\
    \nonumber &+ \left ( \frac{2\eta {\rm B}}{w} \right ) ^2 \lambda_{\max} \Big ( \M^\top \M \Big )  \tilde{L}_S(h_t)\\ 
    \nonumber &\leq \Big ( 1 -  a \eta  \Big )\norm{\w_t - \w^*}^2 + b \eta^2 \Big (  \theta^2 +  \tilde{L}_S(h_t) \Big )\\
    &+ \theta \Big ( c \eta^2 + d \eta  \Big )\norm{\w_t-\w^*}  
\end{align}

In the above we have defined,

\[ a := 2\frac{ (1+\alpha)\lambda_{\min}}{S} , ~b := \left ( \frac{2 B}{w} \right )^2\lambda_{\max} ( \M^\top \M) , ~c :=   2b \times \frac{ BL }{w} \Big ( \sum_{i=1}^{w} \sqrt{\lambda_{\max} \Big ( \A_i \A_i^\top \Big )} \Big ) , ~d :=  2 \sqrt{b} \]

Now we note the following upperbound on $\tilde{L}_S$, 

\begin{align*}
    \tilde{L}_S(h_t) &:= \frac{1}{S}\sum_{i=1}^S \Big (f_{\w^*}(\x_i) - f_{\w_t} (\x_i) \Big )^2 = \frac{1}{wS}\sum_{i=1}^S \sum_{j=1}^w \Bigg (\sigma \Big (\langle \A_j^\top \w^*, \x_i \rangle \Big ) - \sigma \Big ( \langle \A_j^\top \w_t, \x_i \rangle \Big ) \Bigg )^2\\
    &\leq \frac{L}{wS}\sum_{i=1}^S \sum_{j=1}^w \vert (\w^* - \w_t)^\top(\A_j \x_i)  \vert ^2 \leq \frac{L}{wS}\sum_{i=1}^S \sum_{j=1}^w \norm{\w^* - \w_t}^2\norm{\A_j \x_i}^2  \\
    &\leq \frac{L}{wS} \times \norm{\w^* - \w_t}^2 \times \sum_{i=1}^S \sum_{j=1}^w \x_i^\top \A_j^\top \A_j \x_i \leq \frac{L}{wS} \times \norm{\w^* - \w_t}^2 \times \sum_{i=1}^S \lambda_{\max} \Big (\sum_{j=1}^w \A_j^\top \A_j \Big ) \norm{\x_i}^2\\ 
    &\leq \frac{B^2L}{w} \times \norm{\w^* - \w_t}^2 \times  \lambda_{\max} \Big (\sum_{j=1}^w \A_j^\top \A_j \Big )
    % &\leq \frac{L}{wS}\sum_{i=1}^S \sum_{j=1}^w \vert (\A_j^\top \w^*)^\top \x_i - (\A_j^\top \w_t)^\top \x_i \vert ^2 \leq \frac{B^2L}{w} \sum_{j=1}^w \norm{   (\w^* - \w_t)^\top \A_j } ^2\\
    % &\leq \frac{B^2L}{w} \sum_{j=1}^w \A_j^\top (\w^* - \w_t)(\w^* - \w_t)^\top \A_j \\
    % &\leq \norm{\w^* - \w_t}^2 \Big (  \frac{L}{w}  \sum_{j=1}^w \norm{\A_j}^2 \Big ) = f \norm{\w^* - \w_t}^2  
\end{align*}

We define, $f :=   \frac{B^2L}{w}  \lambda_{\max} \Big (\sum_{j=1}^w \A_j^\top \A_j \Big )  $ and substituting the above into equation \ref{prefinal} and defining, $\Delta_t = \norm{\w_t - \w^*}$ we have, 

\[ \Delta_{t+1}^2 \leq  (1 - a\eta + b \eta^2 f) \Delta_t^2  + \theta (c \eta^2 + d \eta) \Delta_t + b \eta^2 \theta^2 \]


Now we choose $\eta = \frac{a}{2bf}$ which minimizes the coefficient of $\Delta_t^2$ in the RHS above. And lets define $p := c \Big ( \frac{a}{2bf} \Big )^2+ d \Big ( \frac{a}{2bf} \Big )$ and $q = b \Big ( \frac{a}{2bf} \Big )^2 $. Then the change in the distance from the true parameter can be written as, 

\[ \Delta_{t+1}^2 \leq  \Big (1 - \frac{a^2}{4bf} \Big ) \Delta_t^2  + \theta p \Delta_t + \theta^2 q  \] 


At this point now we specialize to the case in the theorem which corresponds to $\theta =0$.  Then the dynamics of the iterates above can be solved to give for any $T \in \Z^+$, 

\[ \Delta_T^2 \leq  \Big (1 - \frac{a^2}{4bf} \Big )^{T -1} \Delta_1^2 \]

So we can get $\epsilon$ close in $2-$norm to the true weights $\w^*$ in time, $T \leq 1 + \frac{2}{\log \Big [ \frac{1}{1 - \frac{a^2}{4bf}} \Big ]}\log \Big ( \frac{W}{\epsilon} \Big )$ 

Its clear that for the above to be meaningful we need $a^2 < 4bf$ and simplifying that leads to the condition that was imposed in equation \ref{cond1} 


% \paragraph{{\bf Case $1$ : Suppose the data is realizable i.e $\theta =0$}} 
% ~\\
% Then the dynamics of the iterates above can be solved to give for any $T \in \Z^+$, 

% \[ \Delta_T^2 \leq  \Big (1 - \frac{a^2}{4bf} \Big )^{T -1} \Delta_1^2 \]

% So we can get $\epsilon$ close in $2-$norm to the true weights $\w^*$ in time, $T \leq 1 + \frac{2}{\log \Big [ \frac{1}{1 - \frac{a^2}{4bf}} \Big ]}\log \Big ( \frac{W}{\epsilon} \Big )$ 

% Its clear that for the above to be meaningful we need $a^2 < 4bf$ and simplifying that leads to the condition that was imposed in equation \ref{cond1} 

% ~\\
% \paragraph{{\bf Case $2$ : Suppose the data is ``noisily realizable" i.e $\theta > 0$}}


\end{proof}







